Pay Beliefs and the Amenity-Pay Tradeoff

This paper studies how workers' beliefs about pay shape the tradeoffs between pay and workplace amenities. We design a multi-stage incentivized survey experiment that combines hypothetical choice experiments with elicited beliefs about starting salaries in real jobs and randomly varies the provision of explicit pay information. Although stated preferences imply sizable willingness to pay for workplace amenities, baseline beliefs about salaries in real jobs are systematically biased along two margins: respondents under-predict starting salaries by 18% and expect higher-amenity jobs to pay more, substantially over-predicting the amenity-pay gradient. A short-term pay information intervention raises mean beliefs about pay in similar jobs by 4% and reduces belief dispersion by 15%, but does not alter the perceived amenity-pay slope or the implied tradeoffs in stated choices. Meanwhile, full disclosure of pay for jobs under consideration raises the pay of chosen jobs by about 4% and recovers willingness-to-pay estimates closely aligned with full-information hypothetical-choice benchmarks. Short-term disclosure thus moves beliefs but not perceived tradeoffs, while persistent disclosure erases biases in pay beliefs and nearly restores the full-information tradeoffs.

==> raw_files/association_beliefs_amenities.tex <==
Permanent           &      0.0975\sym{***}&      0.0195         &      0.0780\sym{***}&      0.0822\sym{***}&    0.000339         &      0.0819\sym{***}\\
                    &    (0.0217)         &    (0.0248)         &    (0.0291)         &    (0.0156)         &    (0.0203)         &    (0.0241)         \\
Work From Home      &      0.0259         &     -0.0258         &      0.0517         &      0.0203         &     -0.0164         &      0.0367         \\
                    &    (0.0305)         &    (0.0297)         &    (0.0341)         &    (0.0237)         &    (0.0325)         &    (0.0336)         \\
Shift Work          &      -0.121\sym{***}&     -0.0835\sym{**} &     -0.0372         &      -0.115\sym{***}&     -0.0659\sym{**} &     -0.0493         \\
                    &    (0.0157)         &    (0.0332)         &    (0.0354)         &    (0.0174)         &    (0.0314)         &    (0.0355)         \\
Flexible Hours      &      0.0601\sym{***}&      0.0171         &      0.0429         &      0.0408\sym{***}&      0.0119         &      0.0288         \\
                    &    (0.0180)         &    (0.0229)         &    (0.0265)         &    (0.0155)         &    (0.0436)         &    (0.0486)         \\


==> raw_files/association_beliefs_amenities_B1.tex <==
Literature WTPs     &       0.592\sym{***}&       0.175\sym{**} &       0.416\sym{***}&       0.500\sym{***}&      0.0960         &       0.404\sym{***}\\
                    &    (0.0718)         &    (0.0807)         &    (0.0919)         &    (0.0589)         &    (0.0892)         &     (0.103)         \\


==> raw_files/association_beliefs_amenities_B1_slides.tex <==
Literature WTPs      &       0.566\sym{***}   &       0.200\sym{**} &       0.366\sym{***}&       0.476\sym{***} &       0.119         &       0.357\sym{***}\\
                     &    (0.0747)    &    (0.0804)             &    (0.0976)                &    (0.0657)       &    (0.0834)     &     (0.103)         \\


==> raw_files/association_beliefs_amenities_B1_slides1.tex <==
Literature WTPs      &       0.566\sym{***}   &  \color{gray}{       0.200\sym{**} }&      \color{gray}{   0.366\sym{***} }&       0.476\sym{***} &       \color{gray}{  0.119  }       &      \color{gray}{   0.357\sym{***} }\\
                     &    (0.0747)    &  \color{gray}{    (0.0804)  }           &  \color{gray}{    (0.0976)    }            &    (0.0657)       &  \color{gray}{    (0.0834)  }   &   \color{gray}{    (0.103)  }       \\


==> raw_files/association_beliefs_amenities_B2.tex <==
Hypothetical Choice WTPs&       0.720\sym{***}&       0.206\sym{**} &       0.514\sym{***}&       0.606\sym{***}&       0.116         &       0.490\sym{***}\\
                    &    (0.0856)         &    (0.0959)         &     (0.107)         &    (0.0728)         &     (0.115)         &     (0.131)         \\


==> raw_files/association_beliefs_amenities_B2_slides.tex <==
Hypothetical Choice WTPs  &       0.687\sym{***} &       0.241\sym{**}&       0.446\sym{***}&       0.576\sym{***}&       0.150          &       0.426\sym{***}\\
                  &    (0.0902)   &    (0.0958)                 &     (0.115)          &    (0.0825)     &     (0.105)             &     (0.128)         \\


==> raw_files/association_beliefs_amenities_B2_slides1.tex <==
Hypothetical Choice WTPs  &       0.687\sym{***} &     \color{gray}{    0.241\sym{**}}&   \color{gray}{      0.446\sym{***}}&       0.576\sym{***}&       \color{gray}{  0.150 }         &   \color{gray}{      0.426\sym{***}}\\
                  &    (0.0902)   &  \color{gray}{    (0.0958)    }             &   \color{gray}{    (0.115)  }        &    (0.0825)     &   \color{gray}{    (0.105) }             &   \color{gray}{    (0.128) }        \\


==> raw_files/association_beliefs_amenities_B3.tex <==
Subjective WTPs     &       0.724\sym{***}&       0.283\sym{***}&       0.441\sym{***}&       0.615\sym{***}&       0.190\sym{*}  &       0.425\sym{***}\\
                    &    (0.0652)         &     (0.101)         &     (0.110)         &    (0.0603)         &     (0.111)         &     (0.124)         \\


==> raw_files/association_beliefs_amenities_B3_slides.tex <==
Subjective WTPs         &       0.699\sym{***}&       0.306\sym{***} &       0.393\sym{***}&       0.590\sym{***}&       0.213\sym{**}  &       0.377\sym{***}\\
                   &    (0.0711)  &    (0.0993)                 &     (0.114)         &    (0.0679)  &     (0.103)                 &     (0.120)         \\


==> raw_files/association_beliefs_amenities_B3_slides1.tex <==
Subjective WTPs         &       0.699\sym{***}&     \color{gray}{    0.306\sym{***} }&  \color{gray}{       0.393\sym{***}}&       0.590\sym{***}&       \color{gray}{  0.213\sym{**} } &   \color{gray}{      0.377\sym{***} }\\
                   &    (0.0711)  &  \color{gray}{    (0.0993)     }            &   \color{gray}{    (0.114) }        &    (0.0679)  &   \color{gray}{    (0.103)  } &     \color{gray}{  (0.120)   }      \\


==> raw_files/association_beliefs_amenities_slides.tex <==
Permanent           &      0.0945\sym{***}&      0.0225         &      0.0720\sym{**} &      0.0775\sym{***}&     0.00176         &      0.0757\sym{***}\\
                    &    (0.0217)         &    (0.0237)         &    (0.0282)         &    (0.0168)         &    (0.0209)         &    (0.0255)         \\
Work From Home      &      0.0118         &     -0.0155         &      0.0274         &     0.00430         &    -0.00467         &     0.00897         \\
                    &    (0.0338)         &    (0.0288)         &    (0.0348)         &    (0.0285)         &    (0.0329)         &    (0.0364)         \\
Shift Work          &      -0.121\sym{***}&     -0.0793\sym{**} &     -0.0414         &      -0.111\sym{***}&     -0.0630\sym{**} &     -0.0481         \\
                    &    (0.0177)         &    (0.0324)         &    (0.0351)         &    (0.0194)         &    (0.0308)         &    (0.0360)         \\
Flexible Hours      &      0.0585\sym{***}&      0.0233         &      0.0352         &      0.0469\sym{**} &      0.0190         &      0.0279         \\
                    &    (0.0194)         &    (0.0203)         &    (0.0242)         &    (0.0181)         &    (0.0389)         &    (0.0451)         \\
\hline
Observations        &        7060         &        7060         &        7060         &        7060         &        7060         &        7060         \\
Individuals         &         353         &         353         &         353         &         353         &         353         &         353         \\
Controls            &                     &                     &                     &  \checkmark         &  \checkmark         &  \checkmark         \\

==> raw_files/association_beliefs_amenities_slides1.tex <==
Permanent           &      0.0945\sym{***}&     \color{gray}{ 0.0225   }      &   \color{gray}{   0.0720\sym{**}} &      0.0775\sym{***}&       \color{gray}{0.00176}         &     \color{gray}{ 0.0757\sym{***}}\\
                    &    (0.0217)         &   \color{gray}{   (0.0237)      }   &   \color{gray}{ (0.0282)      }   &    (0.0168)         &   \color{gray}{   (0.0209)}         &    \color{gray}{(0.0255)}         \\
Work From Home      &      0.0118         &     \color{gray}{  -0.0155  }       &  \color{gray}{    0.0274   }      &     0.00430         &    \color{gray}{  -0.00467}         &    \color{gray}{ 0.00897    }     \\
                    &    (0.0338)         &     \color{gray}{ (0.0288)   }      &  \color{gray}{  (0.0348)  }       &    (0.0285)         &    \color{gray}{  (0.0329) }        &  \color{gray}{  (0.0364)        } \\
Shift Work          &      -0.121\sym{***}&      \color{gray}{ -0.0793\sym{**} } &   \color{gray}{  -0.0414 }        &      -0.111\sym{***}&   \color{gray}{    -0.0630\sym{**} } &  \color{gray}{   -0.0481  }       \\
                    &    (0.0177)         &     \color{gray}{ (0.0324)   }      &   \color{gray}{ (0.0351)    }     &    (0.0194)         &    \color{gray}{  (0.0308) }        &  \color{gray}{  (0.0360)        } \\
Flexible Hours      &      0.0585\sym{***}&      \color{gray}{  0.0233     }    &   \color{gray}{   0.0352   }      &      0.0469\sym{**} &      \color{gray}{  0.0190 }        &   \color{gray}{   0.0279    }     \\
                    &    (0.0194)         &    \color{gray}{  (0.0203)     }    &  \color{gray}{  (0.0242)   }      &    (0.0181)         &    \color{gray}{  (0.0389) }        &   \color{gray}{ (0.0451)        } \\
\hline
Observations        &        7060         &      \color{gray}{    7060     }    &   \color{gray}{     7060 }        &        7060         &        \color{gray}{  7060 }        &       \color{gray}{ 7060        } \\
Individuals         &         353         &       \color{gray}{    353  }       &    \color{gray}{     353 }        &         353         &        \color{gray}{   353 }        &         \color{gray}{ 353        } \\
Controls            &                     &                     &                     &  \checkmark         & \color{gray}{   \checkmark }         &  \color{gray}{  \checkmark      }   \\

==> raw_files/attrition.tex <==
\midrule
Age of Respondent   &        21.8&        21.8&        21.7&        21.8&        21.8\\
                    &      (3.15)&      (3.15)&      (3.02)&      (3.21)&      (3.08)\\
Male                &        .301&        .304&        .302&        .298&        .294\\
                    &      (.459)&       (.46)&      (.459)&      (.458)&      (.456)\\
Immigrant Background&        .102&        .101&       .0958&        .103&        .097\\
                    &      (.303)&      (.302)&      (.294)&      (.304)&      (.296)\\
Year in Programme   &        2.53&        2.53&        2.52&        2.55&        2.55\\
                    &         (2)&      (1.99)&      (1.99)&      (2.01)&      (2.01)\\
Years Studied       &        1.71&        1.72&         1.7&        1.76&        1.75\\
                    &      (1.74)&      (1.74)&      (1.74)&      (1.76)&      (1.76)\\
Currently Working   &        .653&        .652&        .647&        .658&        .652\\
                    &      (.476)&      (.477)&      (.478)&      (.475)&      (.477)\\
Ever Worked Full Time&        .356&        .355&         .35&        .351&        .347\\
                    &      (.479)&      (.479)&      (.477)&      (.478)&      (.476)\\
\midrule
Observations        &        1059&        1037&         971&         923&         856\\


==> raw_files/attrition_new.tex <==
\midrule
Age of Respondent   &        21.8&        21.8&        21.7&        21.8&        21.8\\
                    &      (3.15)&      (3.15)&      (3.02)&      (3.21)&      (3.08)\\
Male                &        .301&        .304&        .302&        .298&        .294\\
                    &      (.459)&       (.46)&      (.459)&      (.458)&      (.456)\\
Immigrant Background&        .102&        .101&       .0958&        .103&        .097\\
                    &      (.303)&      (.302)&      (.294)&      (.304)&      (.296)\\
Year in Programme   &        2.53&        2.53&        2.52&        2.55&        2.55\\
                    &         (2)&      (1.99)&      (1.99)&      (2.01)&      (2.01)\\
Years Studied       &        1.71&        1.72&         1.7&        1.76&        1.75\\
                    &      (1.74)&      (1.74)&      (1.74)&      (1.76)&      (1.76)\\
Currently Working   &        .653&        .652&        .647&        .658&        .652\\
                    &      (.476)&      (.477)&      (.478)&      (.475)&      (.477)\\
Ever Worked Full Time&        .356&        .355&         .35&        .351&        .347\\
                    &      (.479)&      (.479)&      (.477)&      (.478)&      (.476)\\
\midrule
Observations        &        1059&        1037&         971&         923&         856\\


==> raw_files/attrition_tests.tex <==
\midrule
Age of Respondent   &     -.00197&     -.00419&      .00152&      -.0027\\
                    &   (.000994)&    (.00208)&    (.00233)&     (.0032)\\
Male                &      .00673&      .00174&      -.0125&       -.014\\
                    &    (.00492)&    (.00997)&     (.0116)&     (.0155)\\
Immigrant Background&      -.0018&      -.0312&       .0123&      -.0204\\
                    &    (.00751)&     (.0154)&     (.0177)&     (.0238)\\
Year in Programme   &    -.000612&     -.00101&     -.00203&     -.00274\\
                    &    (.00141)&    (.00287)&    (.00332)&    (.00444)\\
Years Studied       &        .003&      .00472&      .00671&       .0112\\
                    &    (.00201)&    (.00414)&    (.00469)&    (.00637)\\
Currently Working   &     -.00124&      -.0124&       .0107&     -.00443\\
                    &    (.00484)&    (.00981)&     (.0115)&     (.0153)\\
Ever Worked Full Time&    -.000264&     -.00575&      -.0136&      -.0166\\
                    &    (.00496)&     (.0101)&     (.0118)&     (.0157)\\
\midrule
Observations        &        1059&        1059&        1059&        1059\\
F-statistic         &        .905&        1.86&        1.39&        .951\\
P-value             &        .501&       .0726&        .206&        .466\\


==> raw_files/beliefs_mean_0_x.tex <==
\midrule
Current Wage&       0.112\sym{***}&       0.113\sym{***}&       0.108\sym{***}&       0.108\sym{***}\\
            &    (0.0388)         &    (0.0342)         &    (0.0372)         &    (0.0333)         \\
Permanent   &     0.00514         &   -0.000456         &     0.00435         &    -0.00138         \\
            &    (0.0207)         &    (0.0182)         &    (0.0204)         &    (0.0182)         \\
Work From Home&      0.0261         &      0.0143         &      0.0261         &      0.0139         \\
            &    (0.0321)         &    (0.0288)         &    (0.0321)         &    (0.0289)         \\
Flexible Hours&     -0.0365         &     -0.0281         &     -0.0309         &     -0.0239         \\
            &    (0.0233)         &    (0.0210)         &    (0.0231)         &    (0.0207)         \\
Shift Work  &    -0.00967         &     -0.0124         &     -0.0108         &     -0.0134         \\
            &    (0.0205)         &    (0.0191)         &    (0.0208)         &    (0.0192)         \\
Male        &      0.0590\sym{***}&      0.0585\sym{***}&      0.0532\sym{**} &      0.0537\sym{***}\\
            &    (0.0209)         &    (0.0185)         &    (0.0218)         &    (0.0195)         \\
Age         &    0.000853         &    0.000665         &     0.00139         &     0.00107         \\
            &   (0.00382)         &   (0.00362)         &   (0.00395)         &   (0.00375)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        8333         &        8333         &        8333         &        8333         \\
Individuals &         425         &         425         &         425         &         425         \\
Jobs        &         944         &         944         &         944         &         944         \\


==> raw_files/beliefs_mean_0_zA.tex <==
\midrule
Permanent   &      0.0961\sym{***}&      0.0975\sym{***}&      0.0869\sym{***}&      0.0873\sym{***}\\
            &    (0.0254)         &    (0.0221)         &    (0.0210)         &    (0.0168)         \\
Work From Home&      0.0122         &      0.0171         &      0.0109         &      0.0169         \\
            &    (0.0399)         &    (0.0323)         &    (0.0347)         &    (0.0267)         \\
Shift Work  &      -0.131\sym{***}&      -0.124\sym{***}&      -0.122\sym{***}&      -0.112\sym{***}\\
            &    (0.0221)         &    (0.0182)         &    (0.0244)         &    (0.0200)         \\
Flexible Hours&      0.0613\sym{***}&      0.0646\sym{***}&      0.0455\sym{**} &      0.0488\sym{***}\\
            &    (0.0213)         &    (0.0188)         &    (0.0194)         &    (0.0162)         \\


==> raw_files/beliefs_mean_0_zB.tex <==
\midrule
Amenity Value, Literature&       0.457\sym{***}&       0.465\sym{***}&       0.405\sym{***}&       0.409\sym{***}\\
            &    (0.0716)         &    (0.0606)         &    (0.0668)         &    (0.0519)         \\
Amenity Value, Subjective&       0.756\sym{***}&       0.753\sym{***}&       0.665\sym{***}&       0.653\sym{***}\\
            &    (0.0922)         &    (0.0760)         &    (0.0897)         &    (0.0704)         \\
Amenity Value, HCE&       0.713\sym{***}&       0.722\sym{***}&       0.628\sym{***}&       0.633\sym{***}\\
            &     (0.112)         &    (0.0932)         &     (0.100)         &    (0.0776)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         \\
Occupation $\times$ Sector FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        8333         &        8333         &        8333         &        8333         \\
Individuals &         425         &         425         &         425         &         425         \\
Jobs        &         944         &         944         &         944         &         944         \\


==> raw_files/beliefs_mean_1.tex <==
\midrule
Pay Information Effect&      0.0207         &      0.0210\sym{*}  &      0.0187         &      0.0190         \\
            &    (0.0138)         &    (0.0124)         &    (0.0137)         &    (0.0125)         \\
Control Group Mean&       10.69\sym{***}&       10.69\sym{***}&       10.69\sym{***}&       10.69\sym{***}\\
            &    (0.0131)         &    (0.0126)         &    (0.0130)         &    (0.0126)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        8333         &        8333         &        8333         &        8333         \\
Individuals &         857         &         857         &         857         &         857         \\
Jobs        &        1096         &        1096         &        1096         &        1096         \\


==> raw_files/beliefs_mean_1_x.tex <==
\midrule
Current Wage&       0.112\sym{***}&       0.113\sym{***}&       0.108\sym{***}&       0.108\sym{***}\\
            &    (0.0388)         &    (0.0342)         &    (0.0372)         &    (0.0333)         \\
Permanent   &     0.00514         &   -0.000456         &     0.00435         &    -0.00138         \\
            &    (0.0207)         &    (0.0182)         &    (0.0204)         &    (0.0182)         \\
Work From Home&      0.0261         &      0.0143         &      0.0261         &      0.0139         \\
            &    (0.0321)         &    (0.0288)         &    (0.0321)         &    (0.0289)         \\
Flexible Hours&     -0.0365         &     -0.0281         &     -0.0309         &     -0.0239         \\
            &    (0.0233)         &    (0.0210)         &    (0.0231)         &    (0.0207)         \\
Shift Work  &    -0.00967         &     -0.0124         &     -0.0108         &     -0.0134         \\
            &    (0.0205)         &    (0.0191)         &    (0.0208)         &    (0.0192)         \\
Male        &      0.0590\sym{***}&      0.0585\sym{***}&      0.0532\sym{**} &      0.0537\sym{***}\\
            &    (0.0209)         &    (0.0185)         &    (0.0218)         &    (0.0195)         \\
Age         &    0.000853         &    0.000665         &     0.00139         &     0.00107         \\
            &   (0.00382)         &   (0.00362)         &   (0.00395)         &   (0.00375)         \\
Pay Information Effect&       0.625         &       0.727         &       0.589         &       0.700         \\
            &     (0.524)         &     (0.463)         &     (0.508)         &     (0.458)         \\
Info $\times$ Current Wage&     -0.0547         &     -0.0651         &     -0.0548         &     -0.0658         \\
            &    (0.0516)         &    (0.0457)         &    (0.0505)         &    (0.0454)         \\
Info $\times$ Permanent&     -0.0190         &     -0.0211         &     -0.0255         &     -0.0273         \\
            &    (0.0268)         &    (0.0246)         &    (0.0264)         &    (0.0246)         \\
Info $\times$ Work From Home&     -0.0114         &    0.000683         &     -0.0153         &    -0.00417         \\
            &    (0.0420)         &    (0.0362)         &    (0.0423)         &    (0.0369)         \\
Info $\times$ Flexible Hours&      0.0270         &      0.0148         &      0.0255         &      0.0153         \\
            &    (0.0300)         &    (0.0267)         &    (0.0297)         &    (0.0266)         \\
Info $\times$ Shift Work&    0.000311         &     0.00258         &     0.00443         &     0.00682         \\
            &    (0.0267)         &    (0.0241)         &    (0.0279)         &    (0.0248)         \\
Info $\times$ Male&     -0.0173         &     -0.0221         &     -0.0144         &     -0.0182         \\
            &    (0.0272)         &    (0.0232)         &    (0.0272)         &    (0.0235)         \\
Info $\times$ Age&    -0.00117         &   -0.000771         &    0.000529         &    0.000754         \\
            &   (0.00513)         &   (0.00463)         &   (0.00526)         &   (0.00479)         \\
Info $\times$ Not Employed&     -0.0350         &     -0.0182         &     -0.0406         &     -0.0252         \\
            &    (0.0890)         &    (0.0786)         &    (0.0905)         &    (0.0803)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        8333         &        8333         &        8333         &        8333         \\
Individuals &         857         &         857         &         857         &         857         \\
Jobs        &        1096         &        1096         &        1096         &        1096         \\


==> raw_files/beliefs_mean_1_zA.tex <==
\midrule
Permanent   &      0.0961\sym{***}&      0.0975\sym{***}&      0.0869\sym{***}&      0.0873\sym{***}&                     &                     \\
            &    (0.0254)         &    (0.0221)         &    (0.0210)         &    (0.0168)         &                     &                     \\
Work From Home&      0.0122         &      0.0171         &      0.0109         &      0.0169         &                     &                     \\
            &    (0.0399)         &    (0.0323)         &    (0.0347)         &    (0.0267)         &                     &                     \\
Shift Work  &      -0.131\sym{***}&      -0.124\sym{***}&      -0.122\sym{***}&      -0.112\sym{***}&                     &                     \\
            &    (0.0221)         &    (0.0182)         &    (0.0244)         &    (0.0200)         &                     &                     \\
Flexible Hours&      0.0613\sym{***}&      0.0646\sym{***}&      0.0455\sym{**} &      0.0488\sym{***}&                     &                     \\
            &    (0.0213)         &    (0.0188)         &    (0.0194)         &    (0.0162)         &                     &                     \\
Pay Information Effect&      0.0283         &                     &      0.0324         &                     &      0.0321         &                     \\
            &    (0.0248)         &                     &    (0.0234)         &                     &    (0.0213)         &                     \\
Info $\times$ Permanent&     -0.0111         &     -0.0103         &     -0.0149         &     -0.0143         &     -0.0151         &     -0.0172         \\
            &    (0.0236)         &    (0.0192)         &    (0.0218)         &    (0.0170)         &    (0.0198)         &    (0.0150)         \\
Info $\times$ Work From Home&      0.0381         &      0.0378         &      0.0355         &      0.0352         &      0.0231         &      0.0266         \\
            &    (0.0323)         &    (0.0250)         &    (0.0312)         &    (0.0231)         &    (0.0296)         &    (0.0205)         \\
Info $\times$ Shift Work&      0.0138         &   -0.000788         &      0.0141         &    0.000245         &      0.0221         &     0.00626         \\
            &    (0.0253)         &    (0.0206)         &    (0.0255)         &    (0.0207)         &    (0.0233)         &    (0.0171)         \\
Info $\times$ Flexible Hours&    -0.00364         &     -0.0143         &    -0.00431         &     -0.0148         &    -0.00397         &     -0.0131         \\
            &    (0.0172)         &    (0.0131)         &    (0.0163)         &    (0.0123)         &    (0.0157)         &    (0.0111)         \\


==> raw_files/beliefs_mean_1_zB.tex <==
\midrule
Info $\times$ Amenity Value, Literature&     -0.0111         &     -0.0246         &     -0.0226         &     -0.0363         &     -0.0379         &     -0.0483         \\
            &    (0.0635)         &    (0.0498)         &    (0.0611)         &    (0.0459)         &    (0.0557)         &    (0.0416)         \\
Info $\times$  Amenity Value, Subjective&     -0.0366         &     -0.0219         &     -0.0511         &     -0.0381         &     -0.0843         &     -0.0674         \\
            &    (0.0935)         &    (0.0739)         &    (0.0924)         &    (0.0711)         &    (0.0856)         &    (0.0639)         \\
Info $\times$ Amenity Value, HCE&     -0.0222         &     -0.0274         &     -0.0425         &     -0.0480         &     -0.0670         &     -0.0712         \\
            &     (0.104)         &    (0.0836)         &    (0.0979)         &    (0.0752)         &    (0.0885)         &    (0.0676)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         &                     &$\checkmark$         \\
Occupation $\times$ Sector FE&                     &                     &$\checkmark$         &$\checkmark$         &                     &                     \\
Job FE      &                     &                     &                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&       16841         &       16841         &       16841         &       16841         &       16841         &       16841         \\
Individuals &         857         &         857         &         857         &         857         &         857         &         857         \\
Jobs        &        1096         &        1096         &        1096         &        1096         &        1096         &        1096         \\


==> raw_files/beliefs_var_0_x.tex <==
\midrule
Current Wage&    -0.00902\sym{***}&    -0.00912\sym{***}&    -0.00952\sym{***}&    -0.00950\sym{***}\\
            &   (0.00274)         &   (0.00270)         &   (0.00281)         &   (0.00280)         \\
Permanent   &    -0.00209         &    -0.00179         &    -0.00226         &    -0.00188         \\
            &   (0.00170)         &   (0.00171)         &   (0.00174)         &   (0.00176)         \\
Work From Home&    -0.00243         &    -0.00218         &    -0.00240         &    -0.00228         \\
            &   (0.00263)         &   (0.00272)         &   (0.00272)         &   (0.00277)         \\
Flexible Hours&     0.00346\sym{*}  &     0.00325         &     0.00386\sym{*}  &     0.00358\sym{*}  \\
            &   (0.00203)         &   (0.00202)         &   (0.00210)         &   (0.00209)         \\
Shift Work  &    0.000749         &    0.000538         &     0.00199         &     0.00157         \\
            &   (0.00197)         &   (0.00195)         &   (0.00197)         &   (0.00197)         \\
Male        &   -0.000664         &   -0.000569         &    0.000766         &    0.000884         \\
            &   (0.00193)         &   (0.00195)         &   (0.00193)         &   (0.00195)         \\
Age         &   0.0000499         &  0.00000717         &    0.000219         &    0.000168         \\
            &  (0.000323)         &  (0.000318)         &  (0.000360)         &  (0.000355)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        8333         &        8333         &        8333         &        8333         \\
Individuals &         425         &         425         &         425         &         425         \\
Jobs        &         944         &         944         &         944         &         944         \\


==> raw_files/beliefs_var_0_zA.tex <==
\midrule
Permanent   &    -0.00586\sym{**} &    -0.00489\sym{**} &    -0.00655\sym{***}&    -0.00566\sym{**} \\
            &   (0.00232)         &   (0.00223)         &   (0.00227)         &   (0.00221)         \\
Work From Home&   -0.000126         &   -0.000982         &    0.000205         &   -0.000615         \\
            &   (0.00260)         &   (0.00262)         &   (0.00267)         &   (0.00273)         \\
Shift Work  &     0.00229         &     0.00261         &     0.00207         &     0.00252         \\
            &   (0.00268)         &   (0.00262)         &   (0.00287)         &   (0.00275)         \\
Flexible Hours&    -0.00157         &    -0.00182         &    -0.00202         &    -0.00231         \\
            &   (0.00201)         &   (0.00183)         &   (0.00217)         &   (0.00204)         \\


==> raw_files/beliefs_var_0_zB.tex <==
\midrule
Amenity Value, Literature&     -0.0160\sym{**} &     -0.0161\sym{***}&     -0.0174\sym{**} &     -0.0180\sym{***}\\
            &   (0.00667)         &   (0.00624)         &   (0.00685)         &   (0.00648)         \\
Amenity Value, Subjective&     -0.0246\sym{**} &     -0.0246\sym{**} &     -0.0251\sym{**} &     -0.0258\sym{***}\\
            &    (0.0102)         &   (0.00970)         &    (0.0104)         &   (0.00990)         \\
Amenity Value, HCE&     -0.0289\sym{***}&     -0.0276\sym{***}&     -0.0307\sym{***}&     -0.0302\sym{***}\\
            &    (0.0102)         &   (0.00974)         &    (0.0100)         &   (0.00969)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         \\
Occupation $\times$ Sector FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        8333         &        8333         &        8333         &        8333         \\
Individuals &         425         &         425         &         425         &         425         \\
Jobs        &         944         &         944         &         944         &         944         \\


==> raw_files/beliefs_var_1.tex <==
\midrule
Pay Information Effect&    -0.00305\sym{**} &    -0.00311\sym{***}&    -0.00261\sym{**} &    -0.00275\sym{**} \\
            &   (0.00121)         &   (0.00119)         &   (0.00121)         &   (0.00120)         \\
Control Group Mean&      0.0253\sym{***}&      0.0253\sym{***}&      0.0250\sym{***}&      0.0251\sym{***}\\
            &  (0.000929)         &  (0.000914)         &  (0.000903)         &  (0.000894)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        8333         &        8333         &        8333         &        8333         \\
Individuals &         857         &         857         &         857         &         857         \\
Jobs        &        1096         &        1096         &        1096         &        1096         \\


==> raw_files/beliefs_var_1_x.tex <==
\midrule
Current Wage&    -0.00902\sym{***}&    -0.00912\sym{***}&    -0.00952\sym{***}&    -0.00950\sym{***}\\
            &   (0.00274)         &   (0.00270)         &   (0.00281)         &   (0.00280)         \\
Permanent   &    -0.00209         &    -0.00179         &    -0.00226         &    -0.00188         \\
            &   (0.00170)         &   (0.00171)         &   (0.00174)         &   (0.00176)         \\
Work From Home&    -0.00243         &    -0.00218         &    -0.00240         &    -0.00228         \\
            &   (0.00263)         &   (0.00272)         &   (0.00272)         &   (0.00277)         \\
Flexible Hours&     0.00346\sym{*}  &     0.00325         &     0.00386\sym{*}  &     0.00358\sym{*}  \\
            &   (0.00203)         &   (0.00202)         &   (0.00210)         &   (0.00209)         \\
Shift Work  &    0.000749         &    0.000538         &     0.00199         &     0.00157         \\
            &   (0.00197)         &   (0.00195)         &   (0.00197)         &   (0.00197)         \\
Male        &   -0.000664         &   -0.000569         &    0.000766         &    0.000884         \\
            &   (0.00193)         &   (0.00195)         &   (0.00193)         &   (0.00195)         \\
Age         &   0.0000499         &  0.00000717         &    0.000219         &    0.000168         \\
            &  (0.000323)         &  (0.000318)         &  (0.000360)         &  (0.000355)         \\
Pay Information Effect&     -0.0333         &     -0.0408         &     -0.0418         &     -0.0484         \\
            &    (0.0412)         &    (0.0420)         &    (0.0421)         &    (0.0428)         \\
Info $\times$ Current Wage&     0.00438         &     0.00488         &     0.00550         &     0.00592         \\
            &   (0.00409)         &   (0.00415)         &   (0.00418)         &   (0.00423)         \\
Info $\times$ Permanent&     0.00318         &     0.00262         &     0.00335         &     0.00273         \\
            &   (0.00228)         &   (0.00232)         &   (0.00235)         &   (0.00241)         \\
Info $\times$ Work From Home&     0.00560         &     0.00487         &     0.00645         &     0.00585         \\
            &   (0.00392)         &   (0.00407)         &   (0.00404)         &   (0.00417)         \\
Info $\times$ Flexible Hours&    -0.00254         &    -0.00250         &    -0.00366         &    -0.00353         \\
            &   (0.00280)         &   (0.00281)         &   (0.00287)         &   (0.00289)         \\
Info $\times$ Shift Work&    -0.00134         &    -0.00102         &    -0.00296         &    -0.00246         \\
            &   (0.00253)         &   (0.00256)         &   (0.00249)         &   (0.00257)         \\
Info $\times$ Male&    -0.00117         &    -0.00166         &    -0.00170         &    -0.00227         \\
            &   (0.00260)         &   (0.00256)         &   (0.00267)         &   (0.00263)         \\
Info $\times$ Age&   -0.000719\sym{*}  &   -0.000594         &   -0.000792\sym{**} &   -0.000685\sym{*}  \\
            &  (0.000370)         &  (0.000369)         &  (0.000392)         &  (0.000390)         \\
Info $\times$ Not Employed&    -0.00808         &    -0.00743         &    -0.00562         &    -0.00498         \\
            &   (0.00710)         &   (0.00738)         &   (0.00717)         &   (0.00748)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        8333         &        8333         &        8333         &        8333         \\
Individuals &         857         &         857         &         857         &         857         \\
Jobs        &        1096         &        1096         &        1096         &        1096         \\


==> raw_files/beliefs_var_1_zA.tex <==
\midrule
Permanent   &    -0.00586\sym{**} &    -0.00489\sym{**} &    -0.00655\sym{***}&    -0.00566\sym{**} &                     &                     \\
            &   (0.00232)         &   (0.00223)         &   (0.00227)         &   (0.00221)         &                     &                     \\
Work From Home&   -0.000126         &   -0.000982         &    0.000205         &   -0.000615         &                     &                     \\
            &   (0.00260)         &   (0.00262)         &   (0.00267)         &   (0.00273)         &                     &                     \\
Shift Work  &     0.00229         &     0.00261         &     0.00207         &     0.00252         &                     &                     \\
            &   (0.00268)         &   (0.00262)         &   (0.00287)         &   (0.00275)         &                     &                     \\
Flexible Hours&    -0.00157         &    -0.00182         &    -0.00202         &    -0.00231         &                     &                     \\
            &   (0.00201)         &   (0.00183)         &   (0.00217)         &   (0.00204)         &                     &                     \\
Pay Information Effect&    -0.00251         &                     &    -0.00254         &                     &    -0.00201         &                     \\
            &   (0.00305)         &                     &   (0.00301)         &                     &   (0.00293)         &                     \\
Info $\times$ Permanent&    0.000521         &    -0.00158         &    0.000578         &    -0.00156         &   -0.000129         &    -0.00227         \\
            &   (0.00298)         &   (0.00279)         &   (0.00295)         &   (0.00276)         &   (0.00285)         &   (0.00281)         \\
Info $\times$ Work From Home&    -0.00241         &    -0.00107         &    -0.00268         &    -0.00132         &    -0.00250         &   -0.000554         \\
            &   (0.00303)         &   (0.00310)         &   (0.00301)         &   (0.00308)         &   (0.00320)         &   (0.00326)         \\
Info $\times$ Shift Work&    -0.00587\sym{*}  &    -0.00590\sym{*}  &    -0.00580\sym{*}  &    -0.00582\sym{*}  &    -0.00591\sym{*}  &    -0.00565\sym{*}  \\
            &   (0.00332)         &   (0.00319)         &   (0.00333)         &   (0.00319)         &   (0.00333)         &   (0.00327)         \\
Info $\times$ Flexible Hours&    -0.00181         &   -0.000428         &    -0.00177         &   -0.000412         &    -0.00165         &   -0.000356         \\
            &   (0.00216)         &   (0.00199)         &   (0.00213)         &   (0.00197)         &   (0.00215)         &   (0.00202)         \\


==> raw_files/beliefs_var_1_zB.tex <==
\midrule
Info $\times$ Amenity Value, Literature&   -0.000469         &    0.000797         &   -0.000579         &    0.000600         &    -0.00110         &    0.000166         \\
            &   (0.00768)         &   (0.00712)         &   (0.00769)         &   (0.00709)         &   (0.00754)         &   (0.00704)         \\
Info $\times$  Amenity Value, Subjective&     0.00957         &     0.00914         &     0.00931         &     0.00874         &     0.00870         &     0.00786         \\
            &    (0.0120)         &    (0.0113)         &    (0.0121)         &    (0.0113)         &    (0.0117)         &    (0.0111)         \\
Info $\times$ Amenity Value, HCE&     0.00261         &   0.0000885         &     0.00236         &   -0.000306         &    0.000407         &    -0.00205         \\
            &    (0.0125)         &    (0.0118)         &    (0.0125)         &    (0.0117)         &    (0.0120)         &    (0.0116)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         &                     &$\checkmark$         \\
Occupation $\times$ Sector FE&                     &                     &$\checkmark$         &$\checkmark$         &                     &                     \\
Job FE      &                     &                     &                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&       16841         &       16841         &       16841         &       16841         &       16841         &       16841         \\
Individuals &         857         &         857         &         857         &         857         &         857         &         857         \\
Jobs        &        1096         &        1096         &        1096         &        1096         &        1096         &        1096         \\


==> raw_files/effect_pay_info_amenity_packages.tex <==
\hline
Pay Information Effect&    -0.00257         &    -0.00200         &    -0.00260         \\
                    &   (0.00201)         &   (0.00168)         &   (0.00178)         \\
Expected Effect     &     0.00206\sym{**} &     0.00177\sym{**} &     0.00229\sym{***}\\
                    &  (0.000882)         &  (0.000732)         &  (0.000824)         \\
Difference          &    -0.00463\sym{**} &    -0.00377\sym{**} &    -0.00489\sym{**} \\
                    &   (0.00220)         &   (0.00184)         &   (0.00196)         \\
\hline
Observations        &         705         &         705         &         705         \\
Control Mean        &       0.208         &       0.162         &       0.108         \\


==> raw_files/effects_learning_amenity_outcomes.tex <==
\midrule
Pay Information Effect&   -0.000618         &     0.00133         &    -0.00355         &    -0.00859         \\
            &   (0.00527)         &   (0.00325)         &   (0.00473)         &   (0.00629)         \\
Control Group Mean&       0.867\sym{***}&      0.0535\sym{***}&      0.0835\sym{***}&       0.230\sym{***}\\
            &    (0.0152)         &   (0.00988)         &    (0.0130)         &    (0.0341)         \\
\midrule
Observations&       17140         &       17140         &       17140         &       17140         \\
Individuals &         857         &         857         &         857         &         857         \\
Jobs        &        1167         &        1167         &        1167         &        1167         \\


==> raw_files/effects_learning_amenity_outcomes_oc.tex <==
\midrule
Pay Information Effect&   -0.000529         &      0.0105         &    -0.00221         &    -0.00859         \\
            &   (0.00684)         &   (0.00694)         &   (0.00576)         &   (0.00882)         \\
Control Group Mean&       0.893\sym{***}&      0.0570\sym{***}&      0.0587\sym{***}&       0.267\sym{***}\\
            &    (0.0125)         &    (0.0101)         &   (0.00903)         &    (0.0280)         \\
\midrule
Observations&        9050         &        9050         &        9050         &        9050         \\
Individuals &         905         &         905         &         905         &         905         \\
Jobs        &        1108         &        1108         &        1108         &        1108         \\


==> raw_files/effects_learning_amenity_outcomes_occsector.tex <==
\midrule
Pay Information Effect&    0.000548         &     0.00119         &    -0.00357         &    -0.00156         \\
            &   (0.00511)         &   (0.00344)         &   (0.00419)         &   (0.00461)         \\
Control Group Mean&       0.866\sym{***}&      0.0536\sym{***}&      0.0835\sym{***}&       0.226\sym{***}\\
            &    (0.0132)         &   (0.00925)         &    (0.0118)         &    (0.0295)         \\
\midrule
Observations&       17140         &       17140         &       17140         &       17140         \\
Individuals &         857         &         857         &         857         &         857         \\
Jobs        &        1167         &        1167         &        1167         &        1167         \\


==> raw_files/effects_learning_packages.tex <==
\midrule
Pay Information Effect&   -0.000212         &    -0.00106         &    0.000154         \\
            &   (0.00122)         &   (0.00191)         &   (0.00133)         \\
Control Group Mean&       0.155\sym{***}&       0.189\sym{***}&      0.0957\sym{***}\\
            &   (0.00395)         &   (0.00784)         &   (0.00427)         \\
\midrule
Occupation $\times$ sector FE&                     &                     &                     \\
Observations&       17140         &       17140         &       17140         \\
Individuals &         857         &         857         &         857         \\
Jobs        &        1167         &        1167         &        1167         \\


==> raw_files/effects_learning_packages_oc.tex <==
\midrule
Pay Information Effect&  -0.0000236         &    0.000564         &    0.000636         \\
            &   (0.00270)         &   (0.00171)         &   (0.00172)         \\
Control Group Mean&       0.204\sym{***}&       0.106\sym{***}&       0.167\sym{***}\\
            &   (0.00597)         &   (0.00304)         &   (0.00309)         \\
\midrule
Observations&        9050         &        9050         &        9050         \\
Individuals &         905         &         905         &         905         \\
Jobs        &        1108         &        1108         &        1108         \\


==> raw_files/effects_learning_pay_outcomes.tex <==
\midrule
Pay Information Effect&    -0.00196         &    -0.00199         &      0.0204\sym{*}  &      0.0215\sym{**} \\
            &   (0.00244)         &   (0.00250)         &    (0.0105)         &    (0.0105)         \\
Control Group Mean&       10.81\sym{***}&       10.81\sym{***}&       0.455\sym{***}&       0.454\sym{***}\\
            &    (0.0127)         &    (0.0120)         &    (0.0106)         &    (0.0101)         \\
\midrule
Occupation $\times$ sector FE&                     &$\checkmark$         &                     &$\checkmark$         \\
Observations&       17140         &       17140         &       17140         &       17140         \\
Individuals &         857         &         857         &         857         &         857         \\
Jobs        &        1167         &        1167         &        1167         &        1167         \\


==> raw_files/effects_pay_info_amenity_outcomes.tex <==
\midrule
Pay Information Effect&     0.00241         &     0.00717         &     0.00296         &     -0.0199\sym{*}  \\
            &   (0.00875)         &   (0.00610)         &   (0.00602)         &    (0.0121)         \\
Predicted Effect&  -0.0000440         &    0.000363         &    -0.00402\sym{*}  &     0.00250         \\
            &   (0.00254)         &   (0.00143)         &   (0.00230)         &   (0.00652)         \\
Difference  &     0.00246         &     0.00680         &     0.00699         &     -0.0224\sym{**} \\
            &   (0.00831)         &   (0.00627)         &   (0.00569)         &    (0.0110)         \\
\midrule
Individuals &         857         &         857         &         857         &         857         \\
Jobs        &        1170         &        1170         &        1170         &        1170         \\


==> raw_files/effects_pay_info_amenity_outcomes_oc.tex <==
\midrule
Pay Information Effect&    -0.00219         &      0.0105\sym{*}  &     0.00558         &     -0.0132         \\
            &   (0.00812)         &   (0.00627)         &   (0.00610)         &    (0.0143)         \\
Control Group Mean&       0.895\sym{***}&      0.0559\sym{***}&      0.0578\sym{***}&       0.264\sym{***}\\
            &    (0.0125)         &    (0.0103)         &   (0.00902)         &    (0.0289)         \\
\midrule
Observations&        8730         &        8730         &        8730         &        8730         \\
Individuals &         873         &         873         &         873         &         873         \\
Jobs        &        1099         &        1099         &        1099         &        1099         \\


==> raw_files/effects_pay_info_amenity_packages.tex <==
\midrule
Pay Information Effect&   -0.000285         &    -0.00269         &    -0.00104         \\
            &   (0.00184)         &   (0.00299)         &   (0.00177)         \\
Predicted Effect&    0.000488         &     0.00101         &    0.000937         \\
            &  (0.000613)         &   (0.00131)         &  (0.000666)         \\
Difference  &   -0.000773         &    -0.00370         &    -0.00198         \\
            &   (0.00180)         &   (0.00292)         &   (0.00174)         \\
\midrule
Individuals &         857         &         857         &         857         \\
Jobs        &        1170         &        1170         &        1170         \\


==> raw_files/effects_pay_info_bias.tex <==
\hline
Pay Information Effect&      0.0455\sym{***}&      0.0447\sym{***}&      0.0440\sym{***}&     -0.0236\sym{***}&     -0.0225\sym{***}&     -0.0227\sym{***}\\
                    &    (0.0134)         &    (0.0139)         &    (0.0141)         &   (0.00460)         &   (0.00479)         &   (0.00481)         \\
\hline
Observations        &         705         &         705         &         705         &         705         &         705         &         705         \\
Individual Characteristics&                     &  \checkmark         &  \checkmark         &                     &  \checkmark         &  \checkmark         \\
Job Characteristics &                     &                     &  \checkmark         &                     &                     &  \checkmark         \\
Control Mean        &      -0.132         &      -0.132         &      -0.132         &       0.276         &       0.276         &       0.276         \\


==> raw_files/effects_pay_info_bias_association_amenities_pay.tex <==
\hline
Permanent           &      0.0528\sym{**} &      0.0720\sym{**} &     -0.0192         &      0.0600\sym{**} &      0.0757\sym{***}&     -0.0157         \\
                    &    (0.0252)         &    (0.0282)         &    (0.0160)         &    (0.0240)         &    (0.0255)         &    (0.0156)         \\
Work From Home      &      0.0625\sym{*}  &      0.0274         &      0.0351         &      0.0479         &     0.00897         &      0.0389         \\
                    &    (0.0331)         &    (0.0348)         &    (0.0247)         &    (0.0341)         &    (0.0364)         &    (0.0239)         \\
Shift Work          &     -0.0271         &     -0.0414         &      0.0143         &     -0.0347         &     -0.0481         &      0.0134         \\
                    &    (0.0329)         &    (0.0351)         &    (0.0217)         &    (0.0313)         &    (0.0360)         &    (0.0229)         \\
Flexible Hours      &      0.0223         &      0.0352         &     -0.0129         &      0.0179         &      0.0279         &    -0.00997         \\
                    &    (0.0227)         &    (0.0242)         &    (0.0134)         &    (0.0417)         &    (0.0451)         &    (0.0137)         \\
Constant            &      -0.167\sym{***}&      -0.209\sym{***}&      0.0416\sym{*}  &      -0.211\sym{***}&      -0.263\sym{***}&      0.0519\sym{**} \\
                    &    (0.0344)         &    (0.0373)         &    (0.0232)         &    (0.0372)         &    (0.0382)         &    (0.0262)         \\
\hline
Observations        &        7040         &        7060         &       14100         &        7040         &        7060         &       14100         \\
Ads                 &        1096         &        1079         &        1159         &        1096         &        1079         &        1159         \\
Individuals         &         352         &         353         &         705         &         352         &         353         &         705         \\
Controls            &                     &                     &                     &  \checkmark         &  \checkmark         &  \checkmark         \\


==> raw_files/effects_pay_info_packages.tex <==
\midrule
Pay Information Effect&   -0.000285         &    -0.00269         &    -0.00104         \\
            &   (0.00184)         &   (0.00299)         &   (0.00177)         \\
Predicted Effect&    0.000488         &     0.00101         &    0.000937         \\
            &  (0.000613)         &   (0.00131)         &  (0.000666)         \\
Difference  &   -0.000773         &    -0.00370         &    -0.00198         \\
            &   (0.00180)         &   (0.00292)         &   (0.00174)         \\
\midrule
Individuals &         857         &         857         &         857         \\
Jobs        &        1170         &        1170         &        1170         \\


==> raw_files/effects_pay_info_packages_oc.tex <==
\midrule
Pay Information Effect&    -0.00214         &    -0.00132         &   -0.000515         \\
            &   (0.00332)         &   (0.00183)         &   (0.00189)         \\
Control Group Mean&       0.203\sym{***}&       0.107\sym{***}&       0.164\sym{***}\\
            &   (0.00615)         &   (0.00309)         &   (0.00315)         \\
\midrule
Observations&        8730         &        8730         &        8730         \\
Individuals &         873         &         873         &         873         \\
Jobs        &        1099         &        1099         &        1099         \\


==> raw_files/effects_pay_info_pay_outcomes.tex <==
\midrule
Pay Information Effect&      0.0404\sym{***}&      0.0385\sym{***}&      -0.144\sym{***}&      -0.143\sym{***}\\
            &   (0.00679)         &   (0.00602)         &    (0.0116)         &    (0.0115)         \\
Control Group Mean&       10.82\sym{***}&       10.82\sym{***}&       0.455\sym{***}&       0.455\sym{***}\\
            &    (0.0104)         &    (0.0105)         &    (0.0195)         &    (0.0193)         \\
\midrule
Occupation $\times$ sector FE&                     &$\checkmark$         &                     &$\checkmark$         \\
Observations&        8570         &        8570         &        8570         &        8570         \\
Individuals &         857         &         857         &         857         &         857         \\
Jobs        &        1098         &        1098         &        1098         &        1098         \\


==> raw_files/explaining_jFE.tex <==
Permanent           &      0.0975\sym{***}&      0.0822\sym{***}&     -0.0684         &     -0.0957         \\
                    &    (0.0217)         &    (0.0156)         &    (0.0872)         &    (0.0872)         \\
Work From Home      &      0.0259         &      0.0203         &    -0.00617         &     -0.0211         \\
                    &    (0.0305)         &    (0.0237)         &     (0.151)         &     (0.143)         \\
Shift Work          &      -0.121\sym{***}&      -0.115\sym{***}&      0.0709         &      0.0926         \\
                    &    (0.0157)         &    (0.0174)         &     (0.109)         &     (0.115)         \\
Flexible Hours      &      0.0601\sym{***}&      0.0408\sym{***}&     -0.0797         &     -0.0402         \\
                    &    (0.0180)         &    (0.0155)         &    (0.0754)         &    (0.0814)         \\


==> raw_files/explaining_pFE.tex <==
Current Wage        &       0.118\sym{***}&      -0.558\sym{***}\\
                    &    (0.0408)         &     (0.156)         \\
Currently Permanent &     0.00278         &      0.0843         \\
                    &    (0.0205)         &    (0.0826)         \\
Currently Work From Home&    -0.00248         &      0.0959         \\
                    &    (0.0326)         &     (0.114)         \\
Currently Flexible Hours&     -0.0267         &      0.0969         \\
                    &    (0.0225)         &    (0.0880)         \\
Currrently Shift Work&     -0.0112         &     -0.0209         \\
                    &    (0.0213)         &    (0.0857)         \\
Male                &      0.0596\sym{***}&     -0.0124         \\
                    &    (0.0210)         &    (0.0860)         \\
Age                 &    0.000146         &     -0.0155         \\
                    &   (0.00411)         &    (0.0129)         \\
Currently Not Employed&    -0.00723         &       0.154         \\
                    &    (0.0647)         &     (0.249)         \\


==> raw_files/explainingbias_A.tex <==
\hline
Age of Respondent   &    -0.00354         &   (0.00649)&     0.00103         &   (0.00209)\\
Male                &      0.0893\sym{***}&    (0.0271)&      0.0105         &   (0.00873)\\
Immigrant Background&      0.0268         &    (0.0417)&    -0.00407         &    (0.0134)\\
Year in Programme   &    -0.00597         &    (0.0129)&     0.00582         &   (0.00415)\\
Years Studied       &     0.00792         &    (0.0119)&     0.00117         &   (0.00384)\\
Currently Working   &     0.00189         &    (0.0260)&    -0.00916         &   (0.00837)\\
Ever Worked Full Time&   -0.000997         &    (0.0264)&     0.00202         &   (0.00849)\\
\hline
Observations        &         353         &            &         353         &            \\
Mean Dependent Variable&      -0.132         &            &       0.276         &            \\


==> raw_files/explainingbias_B.tex <==
\hline
Female $\times$ Private Sector $\times$ Education&      -0.244\sym{***}&    (0.0170)&       0.166\sym{***}&   (0.00839)\\
Female $\times$ Private $\times$ Sales/Financial Advisors&      -0.174\sym{***}&    (0.0215)&       0.207\sym{***}&   (0.00998)\\
Female $\times$ Private $\times$ Legal/Research/Social Services&     -0.0805\sym{***}&    (0.0248)&       0.232\sym{***}&    (0.0125)\\
Female $\times$ Private $\times$ Business/Financial Services&      -0.202\sym{***}&    (0.0203)&       0.212\sym{***}&    (0.0122)\\
Female $\times$ Private $\times$ Accountants/HR/Logistics&      -0.190\sym{***}&    (0.0198)&       0.224\sym{***}&    (0.0114)\\
Female $\times$ Public Sector $\times$ Education&      -0.206\sym{***}&    (0.0189)&       0.161\sym{***}&   (0.00828)\\
Female $\times$ Public $\times$ Advisors&      -0.113\sym{***}&    (0.0190)&       0.196\sym{***}&    (0.0108)\\
Female $\times$ Public $\times$ Legal/Research/Social Services&     -0.0233         &    (0.0171)&       0.154\sym{***}&   (0.00818)\\
Female $\times$ Public $\times$ Administration&     -0.0870\sym{***}&    (0.0201)&       0.191\sym{***}&    (0.0107)\\
Female $\times$ Public $\times$ Accountants/HR&      -0.244\sym{***}&    (0.0200)&       0.240\sym{***}&    (0.0130)\\
Male $\times$ Private Sector $\times$ Education&      -0.159\sym{***}&    (0.0266)&       0.137\sym{***}&    (0.0116)\\
Male $\times$ Private $\times$ Sales/Financial Advisors&     -0.0895\sym{***}&    (0.0300)&       0.243\sym{***}&    (0.0168)\\
Male $\times$ Private $\times$ Legal/Research/Social Services&      0.0511\sym{**} &    (0.0255)&       0.209\sym{***}&    (0.0155)\\
Male $\times$ Private $\times$ Business/Financial Services&      -0.123\sym{***}&    (0.0278)&       0.229\sym{***}&    (0.0173)\\
Male $\times$ Private $\times$ Accountants/HR/Logistics&      -0.154\sym{***}&    (0.0295)&       0.225\sym{***}&    (0.0159)\\
Male $\times$ Public Sector $\times$ Education&      -0.119\sym{***}&    (0.0262)&       0.185\sym{***}&    (0.0150)\\
Male $\times$ Public $\times$ Advisors&     0.00598         &    (0.0320)&       0.190\sym{***}&    (0.0193)\\
Male $\times$ Public $\times$ Legal/Research/Social Services&      0.0171         &    (0.0256)&       0.167\sym{***}&    (0.0131)\\
Male $\times$ Public $\times$ Administration&     -0.0523\sym{*}  &    (0.0305)&       0.211\sym{***}&    (0.0145)\\
Male $\times$ Public $\times$ Accountants/HR&      -0.207\sym{***}&    (0.0272)&       0.236\sym{***}&    (0.0184)\\
\hline
Observations&        3530         &            &        3530         &            \\
Individuals &         353         &            &         353         &            \\
Mean Dependent Variable&      -0.132         &            &       0.200         &            \\


==> raw_files/explainingbias_C.tex <==
1.male#23.yrkeskode\_pred#0.public&      -0.159\sym{***}&    (0.0266)&       0.137\sym{***}&    (0.0116)\\
1.male#23.yrkeskode\_pred#1.public&      -0.119\sym{***}&    (0.0262)&       0.185\sym{***}&    (0.0150)\\
1.male#24.yrkeskode\_pred#0.public&     -0.0895\sym{***}&    (0.0300)&       0.243\sym{***}&    (0.0168)\\
1.male#24.yrkeskode\_pred#1.public&     0.00598         &    (0.0320)&       0.190\sym{***}&    (0.0193)\\
1.male#26.yrkeskode\_pred#0.public&      0.0511\sym{**} &    (0.0255)&       0.209\sym{***}&    (0.0155)\\
1.male#26.yrkeskode\_pred#1.public&      0.0171         &    (0.0256)&       0.167\sym{***}&    (0.0131)\\
1.male#33.yrkeskode\_pred#0.public&      -0.123\sym{***}&    (0.0278)&       0.229\sym{***}&    (0.0173)\\
1.male#33.yrkeskode\_pred#1.public&     -0.0523\sym{*}  &    (0.0305)&       0.211\sym{***}&    (0.0145)\\
1.male#43.yrkeskode\_pred#0.public&      -0.154\sym{***}&    (0.0295)&       0.225\sym{***}&    (0.0159)\\
1.male#43.yrkeskode\_pred#1.public&      -0.207\sym{***}&    (0.0272)&       0.236\sym{***}&    (0.0184)\\
\(N\)       &        3530         &            &        3530         &            \\


==> raw_files/explainingbias_slidesB.tex <==
\hline
Female $\times$ Public $\times$ Education&      -0.206\sym{***}&    (0.0189)&       0.161\sym{***}&   (0.00828)\\
Female $\times$ Public $\times$ Advisors&      -0.113\sym{***}&    (0.0190)&       0.196\sym{***}&    (0.0108)\\
Female $\times$ Public $\times$ Legal/Research/Social Services&     -0.0233         &    (0.0171)&       0.154\sym{***}&   (0.00818)\\
Female $\times$ Public $\times$ Administration&     -0.0870\sym{***}&    (0.0201)&       0.191\sym{***}&    (0.0107)\\
Female $\times$ Public $\times$ Accountants/HR&      -0.244\sym{***}&    (0.0200)&       0.240\sym{***}&    (0.0130)\\
Female $\times$ Private $\times$ Education&      -0.244\sym{***}&    (0.0170)&       0.166\sym{***}&   (0.00839)\\
Female $\times$ Private $\times$ Sales/Financial Advisors&      -0.174\sym{***}&    (0.0215)&       0.207\sym{***}&   (0.00998)\\
Female $\times$ Private $\times$ Legal/Research/Social Services&     -0.0805\sym{***}&    (0.0248)&       0.232\sym{***}&    (0.0125)\\
Female $\times$ Private $\times$ Business/Financial Services&      -0.202\sym{***}&    (0.0203)&       0.212\sym{***}&    (0.0122)\\
Female $\times$ Private $\times$ Accountants/HR/Logistics&      -0.190\sym{***}&    (0.0198)&       0.224\sym{***}&    (0.0114)\\
Male $\times$ Public $\times$ Education&      -0.119\sym{***}&    (0.0262)&       0.185\sym{***}&    (0.0150)\\
Male $\times$ Public $\times$ Advisors&     0.00598         &    (0.0320)&       0.190\sym{***}&    (0.0193)\\
Male $\times$ Public $\times$ Legal/Research/Social Services&      0.0171         &    (0.0256)&       0.167\sym{***}&    (0.0131)\\
Male $\times$ Public $\times$ Administration&     -0.0523\sym{*}  &    (0.0305)&       0.211\sym{***}&    (0.0145)\\
Male $\times$ Public $\times$ Accountants/HR&      -0.207\sym{***}&    (0.0272)&       0.236\sym{***}&    (0.0184)\\
Male $\times$ Private $\times$ Education&      -0.159\sym{***}&    (0.0266)&       0.137\sym{***}&    (0.0116)\\
Male $\times$ Private $\times$ Sales/Financial Advisors&     -0.0895\sym{***}&    (0.0300)&       0.243\sym{***}&    (0.0168)\\
Male $\times$ Private $\times$ Legal/Research/Social Services&      0.0511\sym{**} &    (0.0255)&       0.209\sym{***}&    (0.0155)\\
Male $\times$ Private $\times$ Business/Financial Services&      -0.123\sym{***}&    (0.0278)&       0.229\sym{***}&    (0.0173)\\
Male $\times$ Private $\times$ Accountants/HR/Logistics&      -0.154\sym{***}&    (0.0295)&       0.225\sym{***}&    (0.0159)\\
\hline
Observations&        3530         &            &        3530         &            \\
Individuals &         353         &            &         353         &            \\
Mean Dependent Variable&      -0.132         &            &       0.200         &            \\


==> raw_files/hedonic_regressions_actual_pay_workplace_amenities.tex <==
\hline
Permanent           &      0.0979\sym{***}&      0.0447\sym{***}&      0.0332\sym{*}  \\
                    &    (0.0123)         &    (0.0169)         &    (0.0170)         \\
Work From Home      &       0.108\sym{***}&      0.0275\sym{*}  &     0.00956         \\
                    &    (0.0153)         &    (0.0160)         &    (0.0162)         \\
Shift Work          &     -0.0816\sym{***}&     -0.0320\sym{*}  &     -0.0243         \\
                    &    (0.0144)         &    (0.0192)         &    (0.0192)         \\
Flexible Hours      &    -0.00130         &      0.0157         &      0.0423\sym{**} \\
                    &    (0.0155)         &    (0.0155)         &    (0.0168)         \\
\hline
Observations        &        5017         &        1234         &        1234         \\
Controls            &                     &                     &  \checkmark         \\


==> raw_files/heterogeneity1.tex <==
All         &      0.0431\sym{***}&      -0.147\sym{***}&    -0.00569         &     0.00812         &     0.00669         &     -0.0200\sym{*}  &    -0.00489\sym{**} &      0.0455\sym{***}&     -0.0236\sym{***}&         705         \\
            &   (0.00427)         &    (0.0123)         &   (0.00708)         &   (0.00570)         &   (0.00587)         &    (0.0107)         &   (0.00196)         &    (0.0134)         &   (0.00460)         &                     \\


==> raw_files/heterogeneity10.tex <==
Human Geography&      0.0520\sym{***}&      -0.107\sym{**} &      0.0138         &      0.0138         &    -0.00345         &     -0.0448         &    -0.00245         &     0.00998         &     -0.0223         &          58         \\
            &    (0.0160)         &    (0.0446)         &    (0.0245)         &    (0.0215)         &    (0.0231)         &    (0.0412)         &   (0.00700)         &    (0.0437)         &    (0.0147)         &                     \\


==> raw_files/heterogeneity11.tex <==
Other or Interdisciplinary&      0.0314\sym{***}&      -0.123\sym{***}&    -0.00690         &     0.00933         &      0.0136         &     -0.0211         &    -0.00574\sym{**} &      0.0285         &     -0.0241\sym{***}&         272         \\
            &   (0.00667)         &    (0.0196)         &    (0.0114)         &   (0.00933)         &   (0.00965)         &    (0.0166)         &   (0.00281)         &    (0.0220)         &   (0.00751)         &                     \\


==> raw_files/heterogeneity12.tex <==
Political Science&      0.0554\sym{***}&      -0.167\sym{***}&    -0.00281         &     0.00352         &     -0.0183         &     -0.0703\sym{**} &    -0.00391         &      0.0635\sym{*}  &     -0.0143         &          93         \\
            &    (0.0121)         &    (0.0360)         &    (0.0198)         &    (0.0140)         &    (0.0164)         &    (0.0309)         &   (0.00522)         &    (0.0352)         &    (0.0127)         &                     \\


==> raw_files/heterogeneity13.tex <==
Psychology  &      0.0599\sym{***}&      -0.235\sym{***}&     -0.0110         &    -0.00389         &     -0.0122         &      0.0232         &   -0.000783         &      0.0214         &     -0.0344\sym{**} &          71         \\
            &    (0.0126)         &    (0.0398)         &    (0.0196)         &    (0.0158)         &    (0.0197)         &    (0.0304)         &   (0.00571)         &    (0.0467)         &    (0.0136)         &                     \\


==> raw_files/heterogeneity14.tex <==
Sociology   &      0.0536\sym{***}&      -0.163\sym{***}&     -0.0162         &      0.0259         &     0.00828         &     0.00241         &    -0.00415         &      0.0831\sym{*}  &     0.00257         &          59         \\
            &    (0.0134)         &    (0.0434)         &    (0.0217)         &    (0.0198)         &    (0.0171)         &    (0.0450)         &   (0.00629)         &    (0.0494)         &    (0.0159)         &                     \\


==> raw_files/heterogeneity2.tex <==
Males       &      0.0419\sym{***}&      -0.121\sym{***}&   -0.000435         &    -0.00235         &      0.0187\sym{*}  &     -0.0195         &    -0.00737\sym{**} &      0.0289         &     -0.0324\sym{***}&         215         \\
            &   (0.00728)         &    (0.0237)         &    (0.0134)         &    (0.0103)         &   (0.00981)         &    (0.0183)         &   (0.00320)         &    (0.0229)         &   (0.00846)         &                     \\


==> raw_files/heterogeneity3.tex <==
Females     &      0.0436\sym{***}&      -0.158\sym{***}&    -0.00824         &      0.0127\sym{*}  &    0.000537         &     -0.0190         &    -0.00359         &      0.0563\sym{***}&     -0.0197\sym{***}&         490         \\
            &   (0.00527)         &    (0.0143)         &   (0.00835)         &   (0.00685)         &   (0.00724)         &    (0.0131)         &   (0.00232)         &    (0.0162)         &   (0.00549)         &                     \\


==> raw_files/heterogeneity4.tex <==
Ever Worked Full Time&      0.0395\sym{***}&      -0.145\sym{***}&     -0.0172         &     0.00713         &      0.0194\sym{*}  &    -0.00154         &    -0.00732\sym{**} &      0.0433\sym{**} &     -0.0240\sym{***}&         262         \\
            &   (0.00682)         &    (0.0204)         &    (0.0115)         &   (0.00944)         &   (0.01000)         &    (0.0176)         &   (0.00302)         &    (0.0211)         &   (0.00760)         &                     \\


==> raw_files/heterogeneity5.tex <==
Never Worked Full Time&      0.0451\sym{***}&      -0.146\sym{***}&   0.0000839         &     0.00723         &    -0.00128         &     -0.0312\sym{**} &    -0.00360         &      0.0472\sym{***}&     -0.0229\sym{***}&         443         \\
            &   (0.00551)         &    (0.0155)         &   (0.00906)         &   (0.00718)         &   (0.00727)         &    (0.0135)         &   (0.00241)         &    (0.0174)         &   (0.00583)         &                     \\


==> raw_files/heterogeneity6.tex <==
Master Students&      0.0531\sym{***}&      -0.181\sym{***}&     0.00485         &      0.0251         &      0.0491\sym{***}&     -0.0444         &     -0.0129\sym{***}&     0.00271         &     -0.0189         &          83         \\
            &    (0.0114)         &    (0.0348)         &    (0.0202)         &    (0.0161)         &    (0.0153)         &    (0.0316)         &   (0.00495)         &    (0.0297)         &    (0.0127)         &                     \\


==> raw_files/heterogeneity7.tex <==
Bachelor Students&      0.0414\sym{***}&      -0.141\sym{***}&    -0.00728         &     0.00579         &     0.00154         &     -0.0164         &    -0.00391\sym{*}  &      0.0506\sym{***}&     -0.0242\sym{***}&         622         \\
            &   (0.00459)         &    (0.0130)         &   (0.00758)         &   (0.00610)         &   (0.00629)         &    (0.0114)         &   (0.00206)         &    (0.0146)         &   (0.00495)         &                     \\


==> raw_files/heterogeneity8.tex <==
Anthropology&      0.0178         &     -0.0900\sym{*}  &     0.00308         &     -0.0185         &    -0.00308         &     -0.0285         &    -0.00320         &       0.130\sym{**} &     -0.0381\sym{*}  &          46         \\
            &    (0.0209)         &    (0.0451)         &    (0.0315)         &    (0.0274)         &    (0.0261)         &    (0.0424)         &   (0.00795)         &    (0.0524)         &    (0.0210)         &                     \\


==> raw_files/heterogeneity9.tex <==
Economics   &      0.0528\sym{***}&      -0.169\sym{***}&     -0.0106         &      0.0171         &      0.0273\sym{**} &     0.00417         &    -0.00776\sym{*}  &      0.0557\sym{*}  &     -0.0344\sym{***}&         106         \\
            &    (0.0108)         &    (0.0304)         &    (0.0195)         &    (0.0150)         &    (0.0124)         &    (0.0245)         &   (0.00444)         &    (0.0323)         &    (0.0116)         &                     \\


==> raw_files/inverse_hedonic_regs.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{permanent}&\multicolumn{1}{c}{homeoffice}&\multicolumn{1}{c}{shift\_work}&\multicolumn{1}{c}{flextime}\\
\hline
Log wages   &      0.0699         &      0.0791         &      -0.163\sym{**} &       0.124\sym{*}  \\
            &    (0.0762)         &    (0.0677)         &    (0.0716)         &    (0.0642)         \\
\hline
\(N\)       &        1234         &        1234         &        1234         &        1234         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> raw_files/literatureA_backup_feb_22_2026.tex <==
\addlinespace\addlinespace
\multicolumn{10}{l}{\textbf{Permanent position}} \\
\cite{datta2019} & Mixed logit & UK & 2013 & 13 & Permanent position  vs. 1 month & 9.69 & 0.313 & 0.745384615384615 & 0.0240769230769231 & Table 6 \\
\cite{datta2019} & Mixed logit & US & 1871 & 18.4971 & Permanent position  vs. 1 month & 11.13 & 0.422 & 0.601715944661596 & 0.0228143871201432 & Table 6 \\
\cite{datta2019} & Mixed logit & UK & 2013 & 13 & 1 year position vs. 1 month & 6.54 & 0.196 & 0.503076923076923 & 0.0150769230769231 & Table 6 \\
\cite{datta2019} & Mixed logit & US & 1871 & 18.4971 & 1 year position vs. 1 month & 7.88 & 0.275 & 0.426012726319261 & 0.0148671953981976 & Table 6 \\
\cite{mahmud} & Conditional Logit & BD & 23568 & 100 & Permanent position  vs. No contract & 43.5294117647059 & 2.36948298007186 & 0.435294117647059 & 0.0236948298007186 & Table 5 (col 4) \\
\cite{mahmud} & Conditional Logit & BD & 23568 & 100 & 1 year contract  vs. No contract & 26.8627450980392 & 1.51095028041008 & 0.268627450980392 & 0.0151095028041008 & Table 5 (col 4) \\
\cite{mahmud} & Conditional Logit & BD & 23568 & 100 & 6 month contract  vs. No contract & 19.0196078431373 & 1.2702879340295 & 0.190196078431373 & 0.012702879340295 & Table 5 (col 4) \\
\cite{valet2021} & Conditional Logit & DE & 2659 &  & Permament contract vs 2-year &  &  &  &  & S2 Table \\
\addlinespace\addlinespace
\multicolumn{10}{l}{\textbf{Home office}} \\
\cite{datta2019} & Mixed logit & UK & 2013 & 13 & 50\% work from home vs. 0 & 1.87 & 0.199 & 0.232307692307692 & 0.0153076923076923 & Table 6 \\
\cite{datta2019} & Mixed logit & US & 1871 & 18.4971 & 50\% work from home vs. 0 & 3.97 & 0.291 & 0.267609517167556 & 0.015732195857729 & Table 6 \\
\cite{datta2019} & Mixed logit & UK & 2013 & 13 & 100\% work from home vs. 0 & 3.02 & 0.215 & 0.232307692307692 & 0.0165384615384615 & Table 6 \\
\cite{datta2019} & Mixed logit & US & 1871 & 18.4971 & 100\% work from home vs. 0 & 4.95 & 0.321 & 0.267609517167556 & 0.0173540717193506 & Table 6 \\
\cite{drake2023} & Bayesian mixed logit & US & 1500 & 1 & Flexible location & 0.1393 & 0.003 & 0.1393 & 0.003 & Figure 4 \\
\cite{mas2017valuing} & Mixed logit & US & 608 & 17 & Work from home & 1.33 & 0.29 & 0.0782352941176471 & 0.0170588235294118 & Table 5 \\
\cite{nagleretal2022} & Logit & DE & 3307 & 1 & Working from home up to 2 days & 0.055 & 0.00438456632653061 & 0.055 & 0.00438456632653061 & Figure 1 \\
\cite{nagleretal2022} & Logit & DE & 3307 & 1 & Working from home up to 5 days & 0.075 & 0.00454400510204082 & 0.075 & 0.00454400510204082 & Figure 1 \\
\cite{lewandowski2023} & Logit & PL & 11116 & 1 & WFH 2-3 days a week & 0.0513 & 0.00288265306122449 & 0.0513 & 0.00288265306122449 & Table 7 \\
\cite{lewandowski2023} & Logit & PL & 11116 & 1 & WFH 5 days a week & 0.613 & 0.00298469387755102 & 0.613 & 0.00298469387755102 & Table 7 \\
\cite{maestas2023value}  & Mixed logit & US & 1738 & 1 & Telecommute & 0.041 & 0.007 & 0.041 & 0.007 & Table 2 \\
\cite{kesternich} & Logit & NL & 778 & 1 & Telecommute & 0.071 & 0.008 & 0.071 & 0.008 & Table 3 (control) \\
\cite{kesternich} & Logit & NL & 1317 & 1 & Telecommute & 0.039 & 0.005 & 0.039 & 0.005 & Table 4 (control) \\
\cite{derbyshire} & Multinomial logit & UK & 109 & 1 & Working from home ("job involves working from home and does not require travel") & 0.512 & 0.256632653061225 & 0.512 & 0.256632653061225 & Table 5 (no-disability) \\
\cite{landeghem} & Conditional logit & BE & 20396 & 1 & Work from home (at least 1 day) & 0.15 & 0.027 & 0.15 & 0.027 & Table 3 \\
\cite{landeghem} & Conditional logit & BE & 20396 & 1 & Work from home (at least 2 days) & 0.176 & 0.027 & 0.176 & 0.027 & Table 3 \\
\cite{landeghem} & Conditional logit & BE & 20396 & 1 & Work from home ("as much as I want") & 0.197 & 0.027 & 0.197 & 0.027 & Table 3 \\
\addlinespace\addlinespace
\multicolumn{10}{l}{\textbf{Shift work}} \\
\cite{desiere2023} & Nonparametric & BE & 709 & 15 & Morning  shift & -0.56 & 0.22 & -0.0373333333333333 & 0.0146666666666667 & Table 4, median \\
\cite{desiere2023} & Nonparametric & BE & 709 & 15 & Evening shift & -3.36 & 0.26 & -0.224 & 0.0173333333333333 & Table 4, median \\
\cite{desiere2023} & Nonparametric & BE & 709 & 15 & Night shift & -5.42 & 0.49 & -0.361333333333333 & 0.0326666666666667 & Table 4, median \\
\cite{desiere2023} & Nonparametric & BE & 709 & 15 & Rotating - predictable & -3.36 & 0.28 & -0.224 & 0.0186666666666667 & Table 4, median \\
\cite{desiere2023} & Nonparametric & BE & 709 & 15 & Rotating - unpredictable & -5.71 & 0.6 & -0.380666666666667 & 0.04 & Table 4, median \\
\cite{kesternich} & Logit & NL & 778 & 1 & Evening, night or weekend shifts & -0.179 & 0.01 & -0.179 & 0.01 & Table 3 (control) \\
\cite{kesternich} & Logit & NL & 1317 & 1 & Evening, night or weekend shifts & -0.108 & 0.005 & -0.108 & 0.005 & Table 4 (control) \\
\addlinespace\addlinespace
\multicolumn{10}{l}{\textbf{Flexible hours}} \\
\cite{nagleretal2022} & Logit & DE & 3307 & 1 & Flexible schedule & 0.054 & 0.00340136054421769 & 0.054 & 0.00340136054421769 & Figure 1 \\
\cite{drake2023} & Bayesian mixed logit & US & 1500 & 1 & Flexible schedule & 0.0896 & 0.003 & 0.0896 & 0.003 & Figure 4 \\
\cite{mas2017valuing} & Mixed logit & US & 640 & 17 & Flexible schedule & 0.48 & 0.24 & 0.0282352941176471 & 0.0141176470588235 & Table 5 \\
\cite{maestas2023value}  & Mixed logit & US & 1738 & 1 & Set own schedule & 0.088 & 0.007 & 0.088 & 0.007 & Table 2 \\
\cite{kesternich} & Logit & NL & 778 & 1 & Full schedule freedom & 0.109 & 0.012 & 0.109 & 0.012 & Table 3 (control) \\
\cite{kesternich} & Logit & NL & 1317 & 1 & Full schedule freedom & 0.051 & 0.008 & 0.051 & 0.008 & Table 4 (control) \\
\cite{derbyshire} & Multinomial logit & UK & 109 & 1 & Flexible schedule & 0.093 & 0.0596938775510204 & 0.093 & 0.0596938775510204 & Table 5 (no-disability) \\
\cite{bustelo} & Conditional logit & CO & 36651 & 284 & Flexible schedule & 56.65 & 6.45408163265306 & 0.199471830985915 & 0.0227256395515953 & Table 7 (text above for CI) \\
\cite{landeghem} & Conditional logit & BE & 20396 & 1 & Various fixed schedules & 0.223 & 0.018 & 0.223 & 0.018 & Table 3 \\
\cite{landeghem} & Conditional logit & BE & 20396 & 1 & Can ask changes & 0.213 & 0.018 & 0.213 & 0.018 & Table 3 \\
\cite{landeghem} & Conditional logit & BE & 20396 & 1 & Complete flexibility & 0.192 & 0.017 & 0.192 & 0.017 & Table 3 \\
\cite{jost2023} & Linear probability & CH & 1796 & 100 & Flexible schedule & 2.76 & 0.0867102385618638 & 0.0276 & 0.000867102385618638 & Table S7 \\
\addlinespace\addlinespace
\multicolumn{10}{l}{\textbf{Travel time}} \\
\cite{nagleretal2022} & Logit & DE & 3307 & 0.5 & Commuting time (30 vs 15) & -0.053 & 0.00516662361146991 & -0.106 & 0.0103332472229398 & Figure 1 \\
\cite{nagleretal2022} & Logit & DE & 3307 & 1 & Commuting time (45 vs 15) & -0.13 & 0.00532808059932834 & -0.13 & 0.00532808059932834 & Figure 1 \\
\cite{nagleretal2022} & Logit & DE & 3307 & 1.5 & Commuting time (60 vs 15) & -0.22 & 0.00581245156290364 & -0.146666666666667 & 0.00387496770860243 & Figure1 \\
\cite{willen} & Nonparametric & NO & 10008 & 0.6667 & Doubling of commuting time, men & -0.1123 & 0.003395 & -0.168441577921104 & 0.00509224538773061 & Correspondence based on Figure A2 \\
\cite{landeghem} & Conditional logit & BE & 20396 & 1 & Respondent baseline + 15 min, daily & -0.116 & 0.015 & -0.116 & 0.015 & Table 3 \\
\cite{landeghem} & Conditional logit & BE & 20396 & 1 & Respondent baseline - 15 min, daily & 0.09 & 0.015 & 0.09 & 0.015 & Table 3 \\
\cite{labarbanchon} & Admin data & FR & 75071 & 1 & CES of wage and communting time & -0.1345 & 0.0480110664326465 & -0.1345 & 0.0480110664326465 & Table V \\

==> raw_files/literatureA_old.tex <==
    \addlinespace\addlinespace
    \multicolumn{10}{l}{\textbf{Permanent Position}} \\
    \cite{datta2019} & Mixed logit & UK & 2013 & 13 & Permanent position vs. 1 month & 9.690 & 0.313 & 0.745 & 0.024 & Table 6 \\
    \cite{datta2019} & Mixed logit & US & 1871 & 18.4971 & Permanent position vs. 1 month & 11.130 & 0.422 & 0.602 & 0.023 & Table 6 \\
    \cite{datta2019} & Mixed logit & UK & 2013 & 13 & 1 year position vs. 1 month & 6.540 & 0.196 & 0.503 & 0.015 & Table 6 \\
    \cite{datta2019} & Mixed logit & US & 1871 & 18.4971 & 1 year position vs. 1 month & 7.880 & 0.275 & 0.426 & 0.015 & Table 6 \\

    \addlinespace\addlinespace
    \multicolumn{10}{l}{\textbf{Work From Home}} \\
    \cite{datta2019} & Mixed logit & UK & 2013 & 13 & 50\% work from home vs. 0 & 1.870 & 0.199 & 0.232 & 0.015 & Table 6 \\
    \cite{datta2019} & Mixed logit & US & 1871 & 18.4971 & 50\% work from home vs. 0 & 3.970 & 0.291 & 0.268 & 0.016 & Table 6 \\
    \cite{datta2019} & Mixed logit & UK & 2013 & 13 & 100\% work from home vs. 0 & 3.020 & 0.215 & 54.54 & 0.017 & Table 6 \\
    \cite{datta2019} & Mixed logit & US & 1871 & 18.4971 & 100\% work from home vs. 0 & 4.950 & 0.321 & 0.268 & 0.017 & Table 6 \\
    \cite{drake2023} & Bayesian mixed logit & US & 1500 & 1 & Flexible location & 0.139 & 0.003 & 0.139 & 0.003 & Figure 4 \\
    \cite{mas2017valuing} & Mixed logit & US & 608 & 17 & Work from home & 1.330 & 0.290 & 0.078 & 0.017 & table 5 \\
    \cite{nagleretal2022} & Logit & DE & 3307 & 1 & Working from home up to 2 days & 0.055 & 0.004 & 0.055 & 0.004 & Figure 1 \\
    \cite{nagleretal2022} & Logit & DE & 3307 & 1 & Working from home up to 5 days & 0.075 & 0.005 & 0.075 & 0.005 & Figure 1 \\
    \cite{lewandowski2023} & Logit & PL & 11116 & 1 & WFH 2-3 days a week & 0.051 & 0.003 & 0.051 & 0.003 & Table 7 \\
    \cite{lewandowski2023} & Logit & PL & 11116 & 1 & WFH 5 days a week & 0.613 & 0.003 & 0.613 & 0.003 & Table 7 \\
    \cite{maestas2023value} & Mixed logit & US & 1738 & 1 & Telecommute & 0.041 & 0.007 & 0.041 & 0.007 & table 2 \\

    \addlinespace\addlinespace
    \multicolumn{10}{l}{\textbf{Shift Work}} \\
    \cite{desiere2023} & Nonparametric & BE & 709 & 15 & Morning shift & -0.560 & 0.220 & -0.037 & 0.015 & Table 4, median \\
    \cite{desiere2023} & Nonparametric & BE & 709 & 15 & Evening shift & -3.360 & 0.260 & -0.224 & 0.017 & Table 4, median \\
    \cite{desiere2023} & Nonparametric & BE & 709 & 15 & Night shift & -5.420 & 0.490 & -0.361 & 0.033 & Table 4, median \\
    \cite{desiere2023} & Nonparametric & BE & 709 & 15 & Rotating - predictable & -3.360 & 0.280 & -0.224 & 0.019 & Table 4, median \\
    \cite{desiere2023} & Nonparametric & BE & 709 & 15 & Rotating - unpredictable & -5.710 & 0.600 & -0.381 & 0.040 & Table 4, median \\

    \addlinespace\addlinespace
    \multicolumn{10}{l}{\textbf{Flexible Hours}} \\
    \cite{nagleretal2022} & Logit & DE & 3307 & 1 & Flexible schedule & 0.054 & 0.003 & 0.054 & 0.003 & Figure 1 \\
    \cite{drake2023} & Bayesian mixed logit & US & 1500 & 1 & Flexible schedule & 0.090 & 0.003 & 0.090 & 0.003 & Figure 4 \\
    \cite{mas2017valuing} & Mixed logit & US & 640 & 17 & Flexible schedule & 0.480 & 0.240 & 0.028 & 0.014 & Table 5 \\
    \cite{maestas2023value} & Mixed logit & US & 1738 & 1 & Set own schedule & 0.088 & 0.007 & 0.088 & 0.007 & Table 2 \\

    \addlinespace\addlinespace
    \multicolumn{10}{l}{\textbf{Travel Time}} \\
    \cite{nagleretal2022} & Logit & DE & 3307 & 0.5 & Commuting time (30 vs 15) & -0.053 & 0.005 & -0.106 & 0.010 & Figure 1 \\
    \cite{nagleretal2022} & Logit & DE & 3307 & 1 & Commuting time (45 vs 15) & -0.130 & 0.005 & -0.130 & 0.005 & Figure 1 \\
    \cite{nagleretal2022} & Logit & DE & 3307 & 1.50 & Commuting time (60 vs 15) & -0.220 & 0.006 & -0.147 & 0.004 & Figure 1 \\
    \cite{willen} & Nonparametric & NOR & 10008 & 0.67 & Doubling of commuting time (from 20 min) & -0.112 & 0.003 & -0.168 & 0.005 & \makecell{Correspondence\\ based on Fig A2} \\

==> raw_files/literatureB_old.tex <==
\addlinespace
\cite{datta2019}, UK & 0.242 & 0.232 &  &  &  & 2013 & Permanent: Diff. between permanent and 1 yr \\
 & (0.028) & (0.015) &  &  &  &  & \\
\cite{datta2019}, US & 0.176 & 0.268 &  &  &  & 1871 & Home office: Option to work from home 50\% \\
 & (0.027) & (0.016) &  &  &  &  & \\
\cite{drake2023} &  & 0.139 &  & 0.090 &  & 1500 & Flexible schedule, location \\
 &  & (0.003) &  & (0.003) &  &  & \\
\cite{mas2017valuing} &  & 0.078 &  & 0.028 &  & 608 & Work from home, flexible schedule \\
 &  & (0.017) &  & (0.014) &  &  & \\
\cite{nagleretal2022} &  & 0.055 &  &  & -0.128 & 3307 & Work from home up to 2 days \\
 &  & (0.004) &  &  & (0.004) &  & \\
\cite{lewandowski2023} &  & 0.051 &  &  &  & 11116 & Average of WTP at all margins \\
 &  & (0.003) &  &  &  &  & \\
\cite{maestas2023value} &  & 0.041 &  &  &  & 1738 & Telecommute \\
 &  & (0.007) &  &  &  &  & \\
\cite{desiere2023} &  &  & -0.104 &  &  & 709 & Predictable rotating shift - 1/3 night shift \\
 &  &  & (0.022) &  &  &  & \\
\cite{willen} &  &  &  &  & -0.168 & 10008 & \\
 &  &  &  &  & (0.005) &  & \\

        \midrule
Average & 0.209 & 0.124 & -0.104 & 0.059 & -0.148 &  & \\
 & (0.020) & (0.004) & (0.022) & (0.007) & (0.003) &  & \\
Weighted Average & 0.210 & 0.092 & -0.104 & 0.072 & -0.158 &  & \\
 & (0.020) & (0.003) & (0.022) & (0.005) & (0.002) &  & \\
 Inverse-Variance Weighted & 0.208 & 0.088 & -0.104 & 0.087 & -0.144 & & \\ & (0.020) & (0.002) & (0.022) & (0.003) & (0.003) & & \\

==> raw_files/literatureB_slides.tex <==
\addlinespace
Datta (2019), UK & 0.242 & 0.232 &  &  &  & 2013 & Permanent: Difference between permanent and 1 year \\
 & (0.028) & (0.015) &  &  &  &  & \\
Datta (2019), US & 0.176 & 0.268 &  &  &  & 1871 & Work from Home: Option to work from home 50\% \\
 & (0.027) & (0.016) &  &  &  &  & \\
Drake et al. (2023) &  & 0.139 &  & 0.090 &  & 1500 & Flexible schedule, location \\
 &  & (0.003) &  & (0.003) &  &  & \\
Mas and Pallais (2017) &  & 0.078 &  & 0.028 &  & 608 & Work from home, flexible schedule \\
 &  & (0.017) &  & (0.014) &  &  & \\
Nagler et al. (2022) &  & 0.055 &  &  & -0.128 & 3307 & Work from home up to 2 days \\
 &  & (0.004) &  &  & (0.004) &  & \\
Lewandowski et al. (2023) &  & 0.051 &  &  &  & 11116 & Average of WTP at all margins \\
 &  & (0.003) &  &  &  &  & \\
Maestas et al. (2023) &  & 0.041 &  &  &  & 1738 & Telecommute \\
 &  & (0.007) &  &  &  &  & \\
Desiere and Walter (2023) &  &  & -0.104 &  &  & 709 & Predictable rotating shift - 1/3 night shift \\
 &  &  & (0.022) &  &  &  & \\
Butikofer et al. (2024) &  &  &  &  & -0.168 & 10008 & \\
 &  &  &  &  & (0.005) &  & \\

        \midrule
Average & 0.209 & 0.124 & -0.104 & 0.059 & -0.148 &  & \\
 & (0.020) & (0.004) & (0.022) & (0.007) & (0.003) &  & \\
Weighted Average & 0.210 & 0.092 & -0.104 & 0.072 & -0.158 &  & \\
 & (0.020) & (0.003) & (0.022) & (0.005) & (0.002) &  & \\
 Inverse-Variance Weighted Average & 0.208 & 0.088 & -0.104 & 0.087 & -0.144 & & \\ & (0.020) & (0.002) & (0.022) & (0.003) & (0.003) & & \\

==> raw_files/randomization.tex <==
\hline
Age of respondent   &          22&        22.1&        .128&      .00294\\
                    &      (2.99)&      (3.25)&      (.236)&    (.00891)\\
Year in programme   &        2.98&        3.03&       .0513&       .0182\\
                    &      (2.13)&      (2.04)&      (.158)&     (.0207)\\
Years studied       &        2.07&        2.02&      -.0513&      -.0327\\
                    &      (1.88)&      (1.68)&      (.135)&     (.0199)\\
Immigrant background&       .0855&       .0912&       .0057&     .000165\\
                    &       (.28)&      (.288)&     (.0214)&     (.0689)\\
Male                &        .325&        .285&      -.0399&      -.0412\\
                    &      (.469)&      (.452)&     (.0348)&     (.0466)\\
Works currently     &        .689&        .704&       .0142&      .00877\\
                    &      (.463)&      (.457)&     (.0347)&     (.0439)\\
Ever worked FT      &        .333&         .41&       .0769&       .0713\\
                    &      (.472)&      (.493)&     (.0364)&     (.0429)\\


==> raw_files/randomizationA.tex <==
\midrule
Age of Respondent   &        21.7&        21.8&       .0738&    -.000671\\
                    &      (2.99)&      (3.16)&       (.21)&    (.00771)\\
Male                &        .311&        .278&      -.0328&      -.0482\\
                    &      (.463)&      (.448)&     (.0311)&     (.0377)\\
Immigrant Background&       .0965&       .0995&      .00307&      .00666\\
                    &      (.295)&      (.299)&     (.0203)&     (.0569)\\
Year in Programme   &        2.52&        2.57&       .0541&       .0089\\
                    &      (2.04)&      (1.97)&      (.137)&     (.0107)\\
Years Studied       &        1.75&        1.74&     -.00749&      -.0059\\
                    &      (1.81)&      (1.71)&       (.12)&     (.0155)\\
Currently Working   &        .666&        .639&       -.027&      -.0471\\
                    &      (.472)&       (.48)&     (.0325)&     (.0371)\\
Ever Worked Full Time&        .313&         .38&       .0667&       .0864\\
                    &      (.464)&      (.485)&     (.0323)&     (.0379)\\


==> raw_files/randomizationB.tex <==
\midrule
training            &        .641&        .634&     -.00708&       .0236\\
                    &       (.48)&      (.482)&    (.00488)&     (.0127)\\
goodcolleagues      &        .721&        .719&     -.00166&      -.0231\\
                    &      (.449)&       (.45)&     (.0044)&     (.0104)\\
central             &        .616&        .615&     -.00125&     .000121\\
                    &      (.486)&      (.487)&    (.00507)&    (.00702)\\
otherminorperks     &       .0805&       .0826&      .00211&      .00898\\
                    &      (.272)&      (.275)&    (.00287)&    (.00389)\\
permanent           &        .868&        .867&    -.000403&     -.00645\\
                    &      (.339)&      (.339)&    (.00374)&    (.00564)\\
homeoffice          &       .0524&       .0566&      .00424&    -.000696\\
                    &      (.223)&      (.231)&    (.00273)&     (.0061)\\
shift\_work          &       .0841&        .079&     -.00507&      .00192\\
                    &      (.277)&       (.27)&    (.00313)&    (.00572)\\
flextime            &        .222&        .221&     -.00111&       .0145\\
                    &      (.416)&      (.415)&    (.00418)&     (.0104)\\
traveltime          &        2.18&        2.24&       .0628&     -.00138\\
                    &      (1.45)&      (1.44)&     (.0296)&    (.00819)\\
\midrule
Observations        &       17000&       17280&       34280&       34280\\
Individuals         &         425&         432&         857&         857\\
Ads                 &        1167&        1168&        1175&        1175\\
Joint F-statistic   &            &            &            &        1.35\\
P-value             &            &            &            &        .155\\


==> raw_files/robustness1.tex <==
Baseline    &      0.0431\sym{***}&      -0.147\sym{***}&    -0.00569         &     0.00812         &     0.00669         &     -0.0200\sym{*}  &    -0.00489\sym{**} &      0.0455\sym{***}&     -0.0236\sym{***}&         705         \\
            &   (0.00427)         &    (0.0123)         &   (0.00708)         &   (0.00570)         &   (0.00587)         &    (0.0107)         &   (0.00196)         &    (0.0134)         &   (0.00460)         &                     \\


==> raw_files/robustness2.tex <==
Individual controls&      0.0415\sym{***}&      -0.140\sym{***}&    -0.00818         &     0.00567         &     0.00677         &     -0.0211\sym{*}  &    -0.00489\sym{**} &      0.0447\sym{***}&     -0.0225\sym{***}&         705         \\
            &   (0.00442)         &    (0.0127)         &   (0.00733)         &   (0.00589)         &   (0.00600)         &    (0.0111)         &   (0.00196)         &    (0.0139)         &   (0.00479)         &                     \\


==> raw_files/robustness3.tex <==
Individual and job characteristics&      0.0416\sym{***}&      -0.142\sym{***}&    -0.00194         &     0.00129         &     0.00517         &     -0.0138\sym{**} &    -0.00488\sym{**} &      0.0440\sym{***}&     -0.0227\sym{***}&         705         \\
            &   (0.00444)         &    (0.0128)         &   (0.00573)         &   (0.00411)         &   (0.00485)         &   (0.00689)         &   (0.00194)         &    (0.0141)         &   (0.00481)         &                     \\


==> raw_files/robustness4.tex <==
Fatigue controls&      0.0400\sym{***}&      -0.140\sym{***}&    -0.00979         &     0.00471         &      0.0102         &     -0.0202\sym{*}  &    -0.00490\sym{**} &      0.0539\sym{***}&     -0.0259\sym{***}&         705         \\
            &   (0.00481)         &    (0.0137)         &   (0.00797)         &   (0.00642)         &   (0.00661)         &    (0.0120)         &   (0.00197)         &    (0.0151)         &   (0.00518)         &                     \\


==> raw_files/robustness5.tex <==
Time use between 5th and 95th percentile&      0.0434\sym{***}&      -0.147\sym{***}&    -0.00295         &      0.0104\sym{*}  &     0.00408         &     -0.0255\sym{**} &    -0.00429\sym{**} &      0.0482\sym{***}&     -0.0262\sym{***}&         634         \\
            &   (0.00455)         &    (0.0129)         &   (0.00723)         &   (0.00609)         &   (0.00617)         &    (0.0113)         &   (0.00204)         &    (0.0138)         &   (0.00485)         &                     \\


==> raw_files/robustness6.tex <==
Normal time use, fatigue controls&      0.0394\sym{***}&      -0.135\sym{***}&    -0.00784         &     0.00675         &     0.00873         &     -0.0261\sym{**} &    -0.00429\sym{**} &      0.0556\sym{***}&     -0.0289\sym{***}&         634         \\
            &   (0.00512)         &    (0.0144)         &   (0.00815)         &   (0.00687)         &   (0.00696)         &    (0.0128)         &   (0.00204)         &    (0.0155)         &   (0.00548)         &                     \\


==> raw_files/robustnessA.tex <==
Baseline estimates&      0.0801\sym{***}&      -0.147\sym{***}&   -0.000689         &     0.00233         &      0.0143         &     -0.0228\sym{*}  &      0.0455\sym{***}&     -0.0236\sym{***}\\
            &   (0.00650)         &    (0.0123)         &    (0.0113)         &   (0.00982)         &   (0.00945)         &    (0.0136)         &    (0.0134)         &   (0.00460)         \\
\textit{Individuals}           &         705         &         705         &         705         &         705         &         705         &         705         &         705         &         705         \\


==> raw_files/robustnessB.tex <==
Controlling for Fatigue using Quadratic&      0.0768\sym{***}&      -0.140\sym{***}&     -0.0130         &     0.00285         &      0.0174         &     -0.0240         &      0.0539\sym{***}&     -0.0259\sym{***}\\
in Number of Previous Scenarios            &   (0.00727)         &    (0.0137)         &    (0.0127)         &    (0.0111)         &    (0.0106)         &    (0.0153)         &    (0.0151)         &   (0.00518)         \\
\textit{Individuals}           &         705         &         705         &         705         &         705         &         705         &         705         &         705         &         705         \\


==> raw_files/robustnessC.tex <==
Subsample of Individuals with Total Time Use&      0.0800\sym{***}&      -0.147\sym{***}&     0.00321         &     0.00525         &      0.0130         &     -0.0241\sym{*}  &      0.0482\sym{***}&     -0.0262\sym{***}\\
for Survey Within 5th and 95th Percentile            &   (0.00690)         &    (0.0129)         &    (0.0120)         &    (0.0105)         &   (0.00993)         &    (0.0142)         &    (0.0138)         &   (0.00485)         \\
\textit{Individuals}           &         634         &         634         &         634         &         634         &         634         &         634         &         634         &         634         \\


==> raw_files/robustnessD.tex <==
Controlling for Fatigue and Total Time&      0.0749\sym{***}&      -0.135\sym{***}&     -0.0104         &     0.00732         &      0.0164         &     -0.0247         &      0.0556\sym{***}&     -0.0289\sym{***}\\
Use Within 5th and 95th Percentile            &   (0.00775)         &    (0.0144)         &    (0.0135)         &    (0.0118)         &    (0.0112)         &    (0.0161)         &    (0.0155)         &   (0.00548)         \\
\textit{Individuals}           &         634         &         634         &         634         &         634         &         634         &         634         &         634         &         634         \\


==> raw_files/subjective_wtp_details.tex <==
\hline
Permanent           &       0.210\sym{***}&       0.108\sym{***}&       0.158\sym{***}\\
                    &    (0.0197)         &   (0.00276)         &    (0.0117)         \\
Home office         &      0.0925\sym{***}&      0.0739\sym{***}&       0.103\sym{***}\\
                    &   (0.00260)         &   (0.00243)         &   (0.00767)         \\
Shift work          &      -0.104\sym{***}&      -0.196\sym{***}&     -0.0825\sym{***}\\
                    &    (0.0216)         &   (0.00553)         &    (0.0138)         \\
Flexible hours      &      0.0719\sym{***}&      0.0640\sym{***}&      0.0691\sym{***}\\
                    &   (0.00460)         &   (0.00206)         &   (0.00593)         \\
Travel time         &      -0.158\sym{***}&      -0.132\sym{***}&      -0.168\sym{***}\\
                    &   (0.00162)         &   (0.00344)         &   (0.00604)         \\
\hline
Observations        &                     &         742         &       30040         \\
Individuals         &                     &                     &         751         \\


==> raw_files/sumstats_outcomesA.tex <==
\hline
Indicator for Choosing Lowest Paying Job&       .4584&       .3116\\
                    &     [.1565]&     [.1698]\\
                    &     (0.008)&     (0.009)\\
Realized Pay        &       10.82&       10.86\\
                    &    [.05362]&    [.05973]\\
                    &     (0.003)&     (0.003)\\


==> raw_files/sumstats_outcomesA_slides.tex <==
\hline
Mean Pay in Preferred Jobs        &       10.82&       10.86\\
                    &    [.05362]&    [.05973]\\
                    &     (0.003)&     (0.003)\\
Share of Preferred Jobs Having the Lowest Pay&       .4584&       .3116\\
                    &     [.1565]&     [.1698]\\
                    &     (0.008)&     (0.009)\\



==> raw_files/sumstats_outcomesB.tex <==
\hline
Expected Pay        &       10.67&       10.72\\
                    &     [.1949]&     [.1567]\\
                    &     (0.010)&     (0.008)\\
Mean Bias in Pay Beliefs&       -.132&     -.08651\\
                    &     [.1941]&       [.16]\\
                    &     (0.010)&     (0.009)\\
Standard Deviation of Bias in Pay Beliefs&       .2758&       .2522\\
                    &    [.06242]&    [.05977]\\
                    &     (0.003)&     (0.003)\\
\hline
Observations        &         353&         352\\


==> raw_files/tab1.tex <==
\hline
Age of respondent   &        22.2&        22.1&       -.087&     -.00437\\
                    &      (3.27)&      (3.12)&      (.049)&    (.00422)\\
Year in programme   &        3.04&           3&       -.039&     -.00208\\
                    &      (2.09)&      (2.09)&     (.0228)&     (.0103)\\
Years studied       &        2.08&        2.05&      -.0314&      .00686\\
                    &      (1.77)&      (1.78)&     (.0177)&    (.00996)\\
Immigrant background&       .0983&       .0884&     -.00985&      -.0978\\
                    &      (.298)&      (.284)&    (.00446)&     (.0341)\\
Male                &        .306&        .305&     -.00144&     -.00321\\
                    &      (.461)&      (.461)&    (.00503)&     (.0238)\\
Works currently     &          .7&        .697&     -.00368&      -.0145\\
                    &      (.458)&       (.46)&    (.00475)&     (.0225)\\
Ever worked FT      &        .376&        .372&     -.00386&      -.0048\\
                    &      (.485)&      (.484)&    (.00532)&      (.022)\\
\hline
Observations        &         764&         702&         764&         764\\
Percent             &         .37&         .34&            &            \\
Joint F-statistic   &            &            &            &        1.62\\
P-value             &            &            &            &        .128\\


==> raw_files/tab2.tex <==
\hline
Age of respondent   &          21&        21.1&        .107&      .00612\\
                    &      (2.92)&      (3.53)&      (.348)&     (.0119)\\
Year in programme   &         1.9&        1.92&       .0226&        .029\\
                    &      (1.62)&      (1.65)&      (.176)&     (.0214)\\
Years studied       &        1.45&        1.29&       -.158&      -.0444\\
                    &      (1.76)&      (1.61)&      (.181)&     (.0254)\\
Immigrant background&          .1&        .119&        .019&       .0315\\
                    &      (.301)&      (.325)&     (.0336)&       (.09)\\
Male                &        .406&        .351&      -.0544&      -.0467\\
                    &      (.492)&      (.479)&     (.0521)&     (.0579)\\
Works currently     &        .622&        .685&       .0623&       .0729\\
                    &      (.486)&      (.466)&     (.0511)&     (.0587)\\
Ever worked FT      &        .328&        .417&       .0889&       .0876\\
                    &      (.471)&      (.494)&     (.0518)&     (.0604)\\
Log actual wage     &        10.8&        10.8&      -.0037&       -.401\\
                    &     (.0405)&     (.0368)&    (.00415)&      (.714)\\
Permanent           &        .872&         .86&      -.0121&       -.589\\
                    &     (.0755)&     (.0815)&    (.00844)&      (.357)\\
Home office         &       .0947&        .102&      .00766&        .448\\
                    &     (.0674)&     (.0685)&    (.00729)&      (.406)\\
Shift work          &       .0831&       .0845&      .00147&        .252\\
                    &     (.0641)&     (.0607)&    (.00669)&      (.452)\\
Flexible hours      &        .223&        .223&     .000714&        .166\\
                    &     (.0988)&     (.0919)&     (.0102)&      (.319)\\
Exercise program    &        .642&        .625&      -.0172&       -.481\\
                    &     (.0998)&      (.101)&     (.0108)&      (.294)\\
Good colleagues     &        .716&        .725&      .00889&        .407\\
                    &     (.0975)&      (.101)&     (.0107)&      (.297)\\
Central location    &        .612&        .607&     -.00567&       -.244\\
                    &      (.114)&      (.106)&     (.0118)&      (.296)\\
Other minor perks   &       .0892&       .0857&     -.00345&       -.509\\
                    &     (.0558)&     (.0605)&    (.00625)&      (.544)\\
\hline
Observations        &         180&         168&         348&         348\\
F                   &            &            &            &       1.121\\
p                   &            &            &            &       0.334\\


==> raw_files/tab2A.tex <==
\hline
Age of respondent   &          22&        22.1&        .128&      .00292\\
                    &      (2.99)&      (3.25)&      (.236)&    (.00891)\\
Year in programme   &        2.98&        3.03&       .0513&       .0181\\
                    &      (2.13)&      (2.04)&      (.158)&     (.0207)\\
Years studied       &        2.07&        2.02&      -.0513&      -.0327\\
                    &      (1.88)&      (1.68)&      (.135)&     (.0199)\\
Immigrant background&       .0855&       .0914&      .00596&     .000737\\
                    &       (.28)&      (.289)&     (.0215)&     (.0689)\\
Male                &        .325&        .285&      -.0399&      -.0402\\
                    &      (.469)&      (.452)&     (.0348)&     (.0467)\\
Works currently     &        .689&        .704&       .0142&      .00835\\
                    &      (.463)&      (.457)&     (.0347)&     (.0439)\\
Ever worked FT      &        .333&         .41&       .0769&        .072\\
                    &      (.472)&      (.493)&     (.0364)&     (.0429)\\


==> raw_files/tab2B.tex <==
\hline
Log actual wage     &        10.8&        10.8&     -.00282&       -.225\\
                    &       (.04)&       (.04)&    (.00302)&        (.5)\\
On-the-job Training &        .646&        .628&      -.0181&        .288\\
                    &      (.102)&      (.108)&     (.0079)&      (.297)\\
Good colleagues     &        .723&        .719&     -.00413&        .257\\
                    &     (.0985)&      (.103)&    (.00761)&      (.343)\\
Central location    &        .614&        .614&    -.000142&      -.0847\\
                    &      (.113)&      (.111)&    (.00844)&      (.219)\\
Other minor perks   &       .0816&       .0846&      .00299&        .012\\
                    &     (.0565)&     (.0608)&    (.00443)&     (.0269)\\
Permanent           &        .867&        .871&      .00356&        -.56\\
                    &     (.0741)&     (.0784)&    (.00576)&       (.21)\\
Home office         &       .0964&        .101&      .00413&        .109\\
                    &     (.0649)&     (.0693)&    (.00507)&      (.217)\\
Shift work          &       .0791&       .0806&      .00157&        .196\\
                    &     (.0596)&     (.0625)&    (.00461)&      (.207)\\
Flexible hours      &        .227&        .223&     -.00342&        .588\\
                    &     (.0997)&     (.0988)&    (.00749)&      (.384)\\
Travel time         &        2.26&        2.29&       .0326&       .0945\\
                    &      (.688)&      (.768)&      (.055)&      (.264)\\
\hline
Observations        &         351&         351&         702&         701\\
Joint F-statistic   &            &            &            &        1.01\\
p-value             &            &            &            &        .448\\


==> raw_files/tab3.tex <==
\hline
Chose lowest wage job&        .457&        .302&        .487&        .296\\
                    &      (.152)&       (.17)&      (.168)&       (.16)\\
logwage diff, chosen job&       .0273&        .102&      .00826&        .112\\
                    &     (.0876)&     (.0902)&     (.0842)&     (.0846)\\
Log expected wage   &        10.7&           .&        10.7&           .\\
                    &      (.193)&         (.)&      (.168)&         (.)\\
Bias in logs        &       -.126&           .&      -.0924&           .\\
                    &      (.194)&         (.)&      (.171)&         (.)\\
std. dev. of bias in logs&        .278&           .&        .251&           .\\
                    &     (.0634)&         (.)&     (.0626)&         (.)\\
\hline
Observations        &         180&         180&         168&         168\\


==> raw_files/tab3A.tex <==
\hline
Indicator for Choosing Lowest Paying Job &       .4575&        .298&       .4695&       .3117\\
                    &     (.1564)&     (.1738)&      (.159)&     (.1701)\\
Pay Difference Between Chosen and Non-Chosen Job &      .02271&       .1076&      .01376&       .1031\\
                    &    (.08501)&    (.09362)&     (.0858)&    (.08776)\\



==> raw_files/tab3B.tex <==
\hline
Expected Pay   &       10.67&           &       10.72&           \\
                    &     (.1953)&         &     (.1566)&         \\
Mean Bias in Pay Beliefs        &      -.1317&           &     -.08594&           \\
                    &     (.1945)&         &     (.1599)&         \\
Standard Deviation of Bias in Pay Beliefs &       .2758&           &       .2516&           \\
                    &    (.06256)&         &    (.05906)&         \\
\hline
Number of Observations        &         351&         351&         351&         351\\


==> raw_files/tab4.tex <==
\hline
Pay Information Effect   &      0.0851\sym{***}&      0.0869\sym{***}&      0.0861\sym{***}&      -0.160\sym{***}&      -0.159\sym{***}&      -0.162\sym{***}\\
                    &   (0.00925)         &   (0.00976)         &   (0.00989)         &    (0.0167)         &    (0.0175)         &    (0.0179)         \\
\hline
Individual X        &          No         &         Yes         &         Yes         &          No         &         Yes         &         Yes         \\
Job Z               &          No         &          No         &         Yes         &          No         &          No         &         Yes         \\
N                   &         348         &         348         &         348         &         348         &         348         &         348         \\


==> raw_files/tab4A.tex <==
\hline
Pay Information Effect   &      0.0804\sym{***}&      0.0782\sym{***}&      0.0781\sym{***}&      -0.146\sym{***}&      -0.139\sym{***}&      -0.142\sym{***}\\
                    &   (0.00652)         &   (0.00676)         &   (0.00680)         &    (0.0123)         &    (0.0127)         &    (0.0129)         \\
\hline
Individual covariates&          No         &         Yes         &         Yes         &          No         &         Yes         &         Yes         \\
Job characteristics &          No         &          No         &         Yes         &          No         &          No         &         Yes         \\
Observations        &         702         &         701         &         701         &         702         &         701         &         701         \\
Control mean        &        .023         &        .023         &        .023         &         .46         &         .46         &         .46         \\


==> raw_files/tab5.tex <==
\hline
permanent           &      0.0979\sym{***}&      0.0290         &      0.0148         &      0.0257         &     0.00462         &      0.0912\sym{***}&      0.0866\sym{***}&      0.0732\sym{***}\\
                    &    (0.0123)         &    (0.0232)         &    (0.0227)         &    (0.0246)         &    (0.0229)         &    (0.0193)         &    (0.0287)         &    (0.0276)         \\
homeoffice          &       0.108\sym{***}&      0.0370         &      0.0222         &     0.00977         &     0.00405         &      0.0279         &      0.0239         &     0.00448         \\
                    &    (0.0153)         &    (0.0268)         &    (0.0262)         &    (0.0314)         &    (0.0295)         &    (0.0279)         &    (0.0417)         &    (0.0364)         \\
shift\_work          &     -0.0816\sym{***}&     -0.0953\sym{***}&     -0.0750\sym{**} &     -0.0839\sym{**} &     -0.0693\sym{**} &      -0.111\sym{***}&     -0.0414         &     -0.0326         \\
                    &    (0.0144)         &    (0.0332)         &    (0.0325)         &    (0.0363)         &    (0.0340)         &    (0.0235)         &    (0.0406)         &    (0.0337)         \\
flextime            &    -0.00130         &      0.0269         &      0.0368         &      0.0242         &      0.0216         &      0.0405\sym{**} &      0.0189         &     0.00955         \\
                    &    (0.0155)         &    (0.0227)         &    (0.0245)         &    (0.0204)         &    (0.0370)         &    (0.0202)         &    (0.0443)         &    (0.0399)         \\
training            &     -0.0519\sym{***}&      0.0148         &      0.0251         &      0.0208         &      0.0321         &     -0.0117         &     -0.0438         &     -0.0257         \\
                    &    (0.0109)         &    (0.0181)         &    (0.0183)         &    (0.0223)         &    (0.0245)         &    (0.0151)         &    (0.0301)         &    (0.0275)         \\
goodcolleagues      &     -0.0915\sym{***}&     -0.0374\sym{*}  &     -0.0325         &     -0.0392         &     -0.0349         &   0.0000914         &      0.0350         &      0.0174         \\
                    &    (0.0116)         &    (0.0200)         &    (0.0198)         &    (0.0244)         &    (0.0250)         &    (0.0152)         &    (0.0286)         &    (0.0262)         \\
central             &     0.00844         &      0.0339\sym{*}  &      0.0266         &     -0.0160         &     -0.0264         &     -0.0153         &      0.0110         &    0.000901         \\
                    &    (0.0112)         &    (0.0183)         &    (0.0183)         &    (0.0346)         &    (0.0340)         &    (0.0154)         &    (0.0393)         &    (0.0350)         \\
otherminorperks     &     0.00644         &      0.0391         &      0.0237         &     -0.0114         &     -0.0256         &    -0.00632         &      0.0193         &      0.0111         \\
                    &    (0.0195)         &    (0.0323)         &    (0.0318)         &    (0.0439)         &    (0.0371)         &    (0.0263)         &    (0.0471)         &    (0.0389)         \\
\hline
$                   &        5017         &        1234         &        1234         &        3600         &        3600         &        3600         &        3600         &        3360         \\
$                   &                     &                     &                     &         903         &         903         &         903         &         903         &         895         \\
$, ind.             &                     &                     &                     &                     &                     &         180         &         180         &         168         \\
Occup. controls     &                     &                     &         Yes         &                     &         Yes         &         Yes         &         Yes         &         Yes         \\


==> raw_files/tab5A.tex <==
\hline
Permanent           &      0.0938\sym{***}&      0.0218         &      0.0721\sym{**} &      0.0780\sym{***}&     0.00160         &      0.0764\sym{***}\\
                    &    (0.0218)         &    (0.0240)         &    (0.0285)         &    (0.0169)         &    (0.0209)         &    (0.0255)         \\
Home office         &      0.0287         &      0.0115         &      0.0172         &      0.0125         &     0.00863         &     0.00389         \\
                    &    (0.0221)         &    (0.0296)         &    (0.0345)         &    (0.0220)         &    (0.0273)         &    (0.0356)         \\
Shift work          &      -0.119\sym{***}&     -0.0788\sym{**} &     -0.0407         &      -0.110\sym{***}&     -0.0624\sym{**} &     -0.0480         \\
                    &    (0.0177)         &    (0.0322)         &    (0.0351)         &    (0.0194)         &    (0.0305)         &    (0.0360)         \\
Flexible hours      &      0.0573\sym{***}&      0.0209         &      0.0364         &      0.0462\sym{**} &      0.0173         &      0.0289         \\
                    &    (0.0190)         &    (0.0201)         &    (0.0241)         &    (0.0183)         &    (0.0383)         &    (0.0446)         \\
\hline
Observations        &        7020         &        7020         &        7020         &        7020         &        7020         &        7020         \\
Ads                 &        1077         &        1077         &        1077         &        1077         &        1077         &        1077         \\
Individuals         &         351         &                     &         351         &         351         &                     &         351         \\
Occup. controls     &                     &                     &                     &         Yes         &         Yes         &         Yes         \\


==> raw_files/tab5B.tex <==
\hline
Permanent           &      0.0546\sym{**} &      0.0721\sym{**} &     -0.0175         &      0.0618\sym{**} &      0.0764\sym{***}&     -0.0146         \\
                    &    (0.0254)         &    (0.0285)         &    (0.0160)         &    (0.0240)         &    (0.0255)         &    (0.0155)         \\
Home office         &      0.0232         &      0.0172         &     0.00601         &     0.00888         &     0.00389         &     0.00499         \\
                    &    (0.0352)         &    (0.0345)         &    (0.0194)         &    (0.0352)         &    (0.0356)         &    (0.0202)         \\
Shift work          &     -0.0250         &     -0.0407         &      0.0157         &     -0.0342         &     -0.0480         &      0.0138         \\
                    &    (0.0328)         &    (0.0351)         &    (0.0221)         &    (0.0314)         &    (0.0360)         &    (0.0233)         \\
Flexible hours      &      0.0262         &      0.0364         &     -0.0102         &      0.0228         &      0.0289         &    -0.00610         \\
                    &    (0.0230)         &    (0.0241)         &    (0.0133)         &    (0.0409)         &    (0.0446)         &    (0.0138)         \\
Constant            &      -0.171\sym{***}&      -0.210\sym{***}&      0.0397\sym{*}  &      -0.214\sym{***}&      -0.263\sym{***}&      0.0493\sym{*}  \\
                    &    (0.0349)         &    (0.0381)         &    (0.0230)         &    (0.0369)         &    (0.0382)         &    (0.0261)         \\
\hline
Observations        &        7020         &        7020         &       14040         &        7020         &        7020         &       14040         \\
Ads                 &        1093         &        1077         &        1159         &        1093         &        1077         &        1159         \\
Individuals         &         351         &         351         &         702         &         351         &         351         &         702         \\
Occup. controls     &                     &                     &                     &         Yes         &         Yes         &         Yes         \\


==> raw_files/tab6.tex <==
\hline
Permanent           &       0.210         &       0.108\sym{***}&       0.166\sym{***}\\
                    &                  &   (0.00278)         &    (0.0122)         \\
Home office         &      0.0807         &      0.0740\sym{***}&       0.110\sym{***}\\
                    &                  &   (0.00245)         &   (0.00833)         \\
Shift work          &      -0.138         &      -0.195\sym{***}&     -0.0924\sym{***}\\
                    &                  &   (0.00556)         &    (0.0141)         \\
Flexible hours      &      0.0678         &      0.0646\sym{***}&      0.0718\sym{***}\\
                    &                  &   (0.00212)         &   (0.00608)         \\
Travel time (30 mins)&     -0.0510         &      -0.132\sym{***}&      -0.173\sym{***}\\
                    &                  &   (0.00344)         &   (0.00600)         \\
\hline
Observations        &                    &         736         &       29800         \\
Individuals         &                     &          736           &         745         \\


==> raw_files/tab7A.tex <==
\hline
Pay Information Effect  &    2.55e-10         &     0.00342         &      0.0128         &     -0.0225\sym{*}  &     -0.0313         \\
                    &    (0.0113)         &   (0.00985)         &   (0.00945)         &    (0.0136)         &    (0.0485)         \\
Predicted effect    &     0.00562         &     0.00636         &     -0.0131\sym{**} &     0.00996\sym{*}  &                     \\
                    &   (0.00613)         &   (0.00546)         &   (0.00585)         &   (0.00521)         &                     \\
Difference          &    -0.00562         &    -0.00294         &      0.0259\sym{**} &     -0.0325\sym{**} &                     \\
                    &    (0.0129)         &    (0.0113)         &    (0.0111)         &    (0.0146)         &                     \\
Value of Tradeoff (literature)  &    5.35e-11         &    0.000276         &    -0.00177         &    -0.00153\sym{*}  &     0.00159         \\
                    &   (0.00238)         &  (0.000795)         &   (0.00131)         &  (0.000925)         &   (0.00247)         \\
Value of Tradeoff (subjective)   &    2.76e-11         &    0.000253         &    -0.00251         &    -0.00146\sym{*}  &     0.00411         \\
                    &   (0.00122)         &  (0.000729)         &   (0.00185)         &  (0.000882)         &   (0.00638)         \\
Value of Tradeoff (HCE)          &    4.22e-11         &    0.000375         &    -0.00119         &    -0.00162\sym{*}  &     0.00541         \\
                    &   (0.00187)         &   (0.00108)         &  (0.000874)         &  (0.000980)         &   (0.00839)         \\
\hline
Observations individuals&         702         &         702         &         702         &         702         &         702         \\
Observations ads    &        1234         &        1234         &        1234         &        1234         &                     \\


==> raw_files/tab7B.tex <==
\hline
Pay Information Effect              &    -0.00772\sym{*}  &    1.30e-08         &    -0.00653         \\
                    &   (0.00452)         &  (7.93e-08)         &   (0.00409)         \\
Predicted Effect           &     0.00443\sym{**} &    2.24e-08         &     0.00400\sym{**} \\
                    &   (0.00183)         &  (3.19e-08)         &   (0.00163)         \\
Difference          &     -0.0122\sym{**} &   -9.43e-09         &     -0.0105\sym{**} \\
                    &   (0.00488)         &  (8.56e-08)         &   (0.00440)         \\
\hline
Observations, individuals&         348         &         348         &         348         \\
Observations, ads   &        1234         &        1234         &        1234         \\


==> raw_files/tab7C.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{5}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\
            &\multicolumn{1}{c}{Permanent}&\multicolumn{1}{c}{Travel Time}&\multicolumn{1}{c}{Work from Home}&\multicolumn{1}{c}{Shift Work}&\multicolumn{1}{c}{Flexible Hours}\\
\hline
Treated       &    -0.00800         &     -0.0886         &    -0.00750         &      0.0292\sym{**} &  -0.0000529         \\
            &    (0.0158)         &    (0.0656)         &    (0.0131)         &    (0.0138)         &    (0.0196)         \\
[1em]
Sorting     &     -0.0181         &       0.112         &    -0.00340         &       0.282\sym{***}&      -0.620         \\
            &     (0.117)         &     (0.616)         &     (0.196)         &    (0.0931)         &     (0.922)         \\
[1em]
Treated $\times$ Sorting&       0.331\sym{*}  &       0.409         &     -0.0783         &      -0.326\sym{**} &      -2.067         \\
            &     (0.175)         &     (1.054)         &     (0.313)         &     (0.146)         &     (1.339)         \\
[1em]
Control Mean&      0.0564\sym{***}&      -0.192\sym{***}&      0.0265\sym{***}&     -0.0603\sym{***}&      0.0787\sym{***}\\
            &    (0.0109)         &    (0.0452)         &   (0.00902)         &   (0.00954)         &    (0.0136)         \\
[1em]
Value       &     0.00162         &      0.0165         &   -0.000734         &    -0.00485\sym{***}&   -0.000448         \\
            &   (0.00260)         &    (0.0117)         &   (0.00117)         &   (0.00160)         &   (0.00139)         \\
\hline
\(N\)       &         325         &         325         &         325         &         325         &         325         \\
\hline\hline
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{6}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\multicolumn{6}{p{1.3\linewidth}}{\footnotesize 
            \textbf{Notes:} Difference in probability of choosing a job with an amenity depending on treatment and sorting.}\\
\end{tabular}
}


==> raw_files/tab7D.tex <==
\hline
Pay Information Effect              &    -0.00257         &    -0.00359         &    -0.00196         \\
                    &   (0.00333)         &   (0.00287)         &   (0.00268)         \\
Predicted Effect     &     0.00410\sym{**} &     0.00415\sym{***}&     0.00326\sym{**} \\
                    &   (0.00167)         &   (0.00148)         &   (0.00133)         \\
Difference          &    -0.00667\sym{*}  &    -0.00774\sym{**} &    -0.00522\sym{*}  \\
                    &   (0.00372)         &   (0.00322)         &   (0.00299)         \\
\hline
Number of Individuals&         649         &         649         &         649         \\
Number of Ads    &        1234         &        1234         &        1234         \\


==> raw_files/tab7D_short.tex <==
\hline
Pay Information Effect              &   &      &    -0.00672\sym{*}          \\
                    &   &        &   (0.00387)               \\
Predicted Effect     &     & &     0.00411\sym{***} \\
                    &   &       &   (0.00150)                  \\
Difference          &     & &     -0.0108\sym{***}  \\
                    &  &      &   (0.00413)           \\
\hline
Number of Individuals&              &              &         325         \\
Number of Ads    &             &               &        1234         \\


==> raw_files/tab7X.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{Permanent}&\multicolumn{1}{c}{Work from Home}&\multicolumn{1}{c}{Shift Work}&\multicolumn{1}{c}{Flexible Hours}\\
\hline
Actual Pay   &      0.0699         &      0.0791         &      -0.163\sym{**} &       0.124\sym{*}  \\
            &    (0.0762)         &    (0.0677)         &    (0.0716)         &    (0.0642)         \\
\hline
Number of Job Ads       &        1234         &        1234         &        1234         &        1234         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses.}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.1\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> raw_files/tab8.tex <==
\hline
Pay Information Effect &      0.0335\sym{*}  &     -0.0270\sym{***}&     -0.0191\sym{**} &      0.0302\sym{*}  \\
                    &    (0.0196)         &   (0.00676)         &   (0.00922)         &    (0.0171)         \\
Constant            &      -0.126\sym{***}&       0.278\sym{***}&      0.0273\sym{***}&       0.457\sym{***}\\
                    &    (0.0136)         &   (0.00469)         &   (0.00641)         &    (0.0119)         \\
\hline
Number of Observations        &         348         &         348         &         348         &         348         \\


==> raw_files/tab8A-edited.tex <==
\hline
Pay Information Effect  &      0.0510\sym{***}&      0.0531\sym{***}&      0.0558\sym{***}&     -0.0233\sym{***}&     -0.0221\sym{***}&     -0.0216\sym{***}\\
                    &    (0.0140)         &    (0.0158)         &    (0.0176)         &   (0.00478)         &   (0.00549)         &   (0.00611)         \\
\hline
Control Dependent Mean            &      \multicolumn{3}{c}{-0.130}        &      \multicolumn{3}{c}{0.275}\\
\hline
Observations        &         649       &         572         &         572         &         649         &         572         &         572          \\
Baseline Controls           &          No         &         Yes         &         Yes         &          No         &         Yes         &         Yes         \\
Fatigue Controls   &          No         &          No         &         Yes         &          No         &          No         &         Yes         \\


==> raw_files/tab8A.tex <==
\hline
Wage transparency   &      0.0457\sym{***}&      0.0436\sym{***}&      0.0493\sym{***}&     -0.0242\sym{***}&     -0.0231\sym{***}&     -0.0234\sym{***}\\
                    &    (0.0134)         &    (0.0141)         &    (0.0158)         &   (0.00459)         &   (0.00479)         &   (0.00538)         \\
\hline
Control group mean  &      -0.132         &      -0.132         &      -0.132         &       0.276         &       0.276         &       0.276         \\
Observations        &         702         &         701         &         701         &         702         &         701         &         701         \\
Controls            &          No         &         Yes         &         Yes         &          No         &         Yes         &         Yes         \\
Fatigue controls    &          No         &          No         &         Yes         &          No         &          No         &         Yes         \\


==> raw_files/tab8B.tex <==
\hline
Pay Information Effect   &     -0.0191\sym{**} &      0.0302\sym{*}  &    -0.00840\sym{*}  &    -0.00650\sym{*}  &    -0.00806\sym{**} \\
                    &   (0.00922)         &    (0.0171)         &   (0.00434)         &   (0.00375)         &   (0.00405)         \\
Constant            &      0.0273\sym{***}&       0.457\sym{***}&                     &                     &                     \\
                    &   (0.00641)         &    (0.0119)         &                     &                     &                     \\
\hline
Observations        &         348         &         348         &         348         &         348         &         348         \\


==> raw_files/tabA3.tex <==
\hline
permanent diff, chosen job&       .0611&       .0361&       .0381&       .0494\\
                    &      (.136)&      (.147)&      (.151)&      (.153)\\
homeoffice diff, chosen job&        .025&       .0189&      .00714&        .019\\
                    &      (.111)&      (.132)&      (.145)&      (.127)\\
shift\_work diff, chosen job&      -.0594&      -.0383&      -.0524&      -.0286\\
                    &      (.128)&      (.119)&       (.12)&      (.123)\\
flextime diff, chosen job&       .0772&       .0361&       .0595&       .0696\\
                    &      (.174)&      (.173)&      (.183)&      (.186)\\
traveltime diff, chosen job&       -.198&       -.227&       -.295&       -.271\\
                    &      (.563)&      (.538)&      (.602)&      (.603)\\
training diff, chosen job&     -.00833&       .0139&      -.0696&     -.00655\\
                    &      (.236)&       (.21)&      (.233)&      (.214)\\
goodcolleagues diff, chosen job&       .0211&       .0261&       .0298&        .019\\
                    &      (.204)&        (.2)&      (.213)&      (.194)\\
central diff, chosen job&      .00778&     -.00944&     -.00714&     -.00833\\
                    &      (.213)&      (.211)&      (.217)&       (.22)\\
otherminorperks diff, chosen job&     .000556&     -.00333&     -.00238&     -.00238\\
                    &      (.138)&      (.115)&      (.133)&      (.139)\\
\hline
Observations        &         180&         180&         168&         168\\


==> raw_files/tabXA.tex <==
\hline
Actual Pay  &       0.202\sym{***}&       0.272\sym{***}&       0.172\sym{***}\\
            &    (0.0597)         &    (0.0718)         &    (0.0576)         \\
Own Pay in Last Job&       0.128\sym{***}&       0.157\sym{**} &       0.112\sym{**} \\
            &    (0.0403)         &    (0.0652)         &    (0.0480)         \\
Constant    &       7.163\sym{***}&       6.147\sym{***}&       7.643\sym{***}\\
            &     (0.751)         &     (0.977)         &     (0.776)         \\
\hline
Observations&        6840         &        2120         &        4720         \\
Individuals &         342         &         106         &         236         \\
Job Ads     &        1073         &         758         &         993         \\


==> raw_files/tabXA_slides.tex <==
\hline
Constant Term   &       \color{black}{7.163\sym{***}}&     \color{gray}{  6.147\sym{***} }&   \color{gray}{    7.643\sym{***} }\\
            &     \color{black}{(0.751)}         &  \color{gray}{   (0.977)  }       &  \color{gray}{   (0.776) }        \\
Actual Pay (Job Ad) &       \color{black}{0.202\sym{***}}&      \color{gray}{0.272\sym{***}}&       \color{gray}{0.172\sym{***}}\\
            &   \color{black}{ (0.0597)   }      &   \color{gray}{ (0.0718) }         &  \color{gray}{  (0.0576) }         \\
Own Pay (Last Job) &     \color{black}{  0.128\sym{***}}&    \color{gray}{   0.157\sym{**} }&     \color{gray}{  0.112\sym{**} }\\
            &  \color{black}{  (0.0403) }        &   \color{gray}{ (0.0652) }        &   \color{gray}{ (0.0480)  }       \\
\hline
Individuals &       \color{black}{  342 }        &       \color{gray}{  106  }       &       \color{gray}{  236   }      \\ 
Observations&      \color{black}{  6,840}         &    \color{gray}{    2,120   }      &     \color{gray}{   4,720   }      \\


==> raw_files/tabXB.tex <==
\hline
Actual Pay  &       0.202\sym{***}&       0.272\sym{***}&       0.172\sym{***}\\
            &    (0.0596)         &    (0.0717)         &    (0.0575)         \\
Own Pay in Last Job&       0.128\sym{***}&       0.157\sym{**} &       0.112\sym{**} \\
            &    (0.0403)         &    (0.0651)         &    (0.0479)         \\
Pay Information&       0.903         &       2.070\sym{**} &       0.465         \\
            &     (0.592)         &     (0.865)         &     (0.730)         \\
Pay information $\times$ Actual Pay&     -0.0146         &     -0.0715\sym{*}  &      0.0116         \\
            &    (0.0266)         &    (0.0411)         &    (0.0309)         \\
Pay Information $\times$ Own Pay&     -0.0675         &      -0.122         &     -0.0517         \\
            &    (0.0516)         &    (0.0762)         &    (0.0652)         \\
Constant    &       7.163\sym{***}&       6.147\sym{***}&       7.643\sym{***}\\
            &     (0.751)         &     (0.975)         &     (0.775)         \\
\hline
Observations&       13660         &        4060         &        9600         \\
Individuals &         683         &         203         &         480         \\
Job Ads     &        1158         &         961         &        1136         \\


==> raw_files/tabXB_slides.tex <==
\hline
Constant Term    &       7.163\sym{***}&       6.147\sym{***}&       7.643\sym{***}\\
            &     (0.751)         &     (0.975)         &     (0.775)         \\
Actual Pay  (Job Ad) &       0.202\sym{***}&       0.272\sym{***}&       0.172\sym{***}\\
            &    (0.0596)         &    (0.0717)         &    (0.0575)         \\
Own Pay (Last Job) &       0.128\sym{***}&       0.157\sym{**} &       0.112\sym{**} \\
            &    (0.0403)         &    (0.0651)         &    (0.0479)         \\
Pay Information &       0.903         &       2.070\sym{**} &       0.465         \\
            &     (0.592)         &     (0.865)         &     (0.730)         \\
Pay information $\times$ Actual Pay&     -0.0146         &     -0.0715\sym{*}  &      0.0116         \\
            &    (0.0266)         &    (0.0411)         &    (0.0309)         \\
Pay Information $\times$ Own Pay&     -0.0675         &      -0.122         &     -0.0517         \\
            &    (0.0516)         &    (0.0762)         &    (0.0652)         \\

\hline
Individuals &         683         &         203         &         480         \\
Observations&       13,660         &        4,060         &        9,600         \\

==> raw_files/tab_belief_x_0.tex <==
\midrule
Current Wage&       0.109\sym{***}&       0.110\sym{***}&       0.104\sym{***}&       0.104\sym{***}\\
            &    (0.0324)         &    (0.0305)         &    (0.0317)         &    (0.0300)         \\
Permanent   &     0.00188         &    -0.00227         &     0.00352         &    -0.00108         \\
            &    (0.0179)         &    (0.0167)         &    (0.0176)         &    (0.0165)         \\
Work From Home&     0.00954         &     0.00244         &      0.0113         &     0.00420         \\
            &    (0.0296)         &    (0.0280)         &    (0.0302)         &    (0.0282)         \\
Flexible Hours&     -0.0374\sym{*}  &     -0.0313\sym{*}  &     -0.0319         &     -0.0275         \\
            &    (0.0199)         &    (0.0185)         &    (0.0200)         &    (0.0187)         \\
Shift Work  &     0.00615         &     0.00309         &     0.00301         &    0.000893         \\
            &    (0.0185)         &    (0.0175)         &    (0.0184)         &    (0.0174)         \\
Male        &      0.0547\sym{***}&      0.0555\sym{***}&      0.0509\sym{***}&      0.0525\sym{***}\\
            &    (0.0185)         &    (0.0171)         &    (0.0197)         &    (0.0183)         \\
Age         &   0.0000597         &   -0.000415         &    0.000408         &  -0.0000293         \\
            &   (0.00366)         &   (0.00349)         &   (0.00383)         &   (0.00368)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        9466         &        9466         &        9466         &        9466         \\
Individuals &         480         &         480         &         480         &         480         \\
Jobs        &         994         &         994         &         994         &         994         \\


==> raw_files/tab_belief_x_0_var.tex <==
\midrule
Current Wage&       0.751\sym{*}  &       0.750\sym{**} &       0.760\sym{*}  &       0.758\sym{*}  \\
            &     (0.123)         &     (0.107)         &     (0.123)         &     (0.121)         \\
Permanent   &       0.960         &       0.965         &       0.958         &       0.965         \\
            &    (0.0699)         &    (0.0736)         &    (0.0662)         &    (0.0688)         \\
Work From Home&       1.013         &       1.001         &       1.041         &       1.027         \\
            &     (0.115)         &     (0.116)         &     (0.123)         &     (0.121)         \\
Flexible Hours&       1.134         &       1.130         &       1.141         &       1.135         \\
            &    (0.0935)         &    (0.0930)         &    (0.0997)         &    (0.0900)         \\
Shift Work  &       1.030         &       1.022         &       1.074         &       1.057         \\
            &    (0.0841)         &    (0.0764)         &    (0.0915)         &    (0.0828)         \\
Male        &       1.029         &       1.033         &       1.091         &       1.100         \\
            &    (0.0849)         &    (0.0837)         &     (0.100)         &    (0.0895)         \\
Age         &       1.003         &       1.001         &       1.011         &       1.009         \\
            &    (0.0137)         &    (0.0131)         &    (0.0159)         &    (0.0151)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        9466         &        9466         &        9466         &        9466         \\
Individuals &         480         &         480         &         480         &         480         \\
Jobs        &         994         &         994         &         994         &         994         \\


==> raw_files/tab_belief_x_1.tex <==
\midrule
Current Wage&       0.109\sym{***}&       0.110\sym{***}&       0.104\sym{***}&       0.104\sym{***}\\
            &    (0.0324)         &    (0.0305)         &    (0.0317)         &    (0.0300)         \\
Permanent   &     0.00188         &    -0.00227         &     0.00352         &    -0.00108         \\
            &    (0.0179)         &    (0.0167)         &    (0.0176)         &    (0.0165)         \\
Work From Home&     0.00954         &     0.00244         &      0.0113         &     0.00420         \\
            &    (0.0296)         &    (0.0280)         &    (0.0302)         &    (0.0282)         \\
Flexible Hours&     -0.0374\sym{*}  &     -0.0313\sym{*}  &     -0.0319         &     -0.0275         \\
            &    (0.0199)         &    (0.0185)         &    (0.0200)         &    (0.0187)         \\
Shift Work  &     0.00615         &     0.00309         &     0.00301         &    0.000893         \\
            &    (0.0185)         &    (0.0175)         &    (0.0184)         &    (0.0174)         \\
Male        &      0.0547\sym{***}&      0.0555\sym{***}&      0.0509\sym{***}&      0.0525\sym{***}\\
            &    (0.0185)         &    (0.0171)         &    (0.0197)         &    (0.0183)         \\
Age         &   0.0000597         &   -0.000415         &    0.000408         &  -0.0000293         \\
            &   (0.00366)         &   (0.00349)         &   (0.00383)         &   (0.00368)         \\
Pay Information Effect&       0.548         &       0.595         &       0.533         &       0.589         \\
            &     (0.445)         &     (0.415)         &     (0.438)         &     (0.409)         \\
Info $\times$ Own Wage&     -0.0493         &     -0.0551         &     -0.0511         &     -0.0572         \\
            &    (0.0441)         &    (0.0412)         &    (0.0433)         &    (0.0405)         \\
Info $\times$ Permanent&     -0.0295         &     -0.0320         &     -0.0359         &     -0.0380\sym{*}  \\
            &    (0.0235)         &    (0.0220)         &    (0.0235)         &    (0.0220)         \\
Info $\times$ Work From Home&    -0.00536         &     0.00340         &     -0.0108         &    -0.00203         \\
            &    (0.0373)         &    (0.0347)         &    (0.0380)         &    (0.0350)         \\
Info $\times$ Flexible Hours&      0.0376         &      0.0294         &      0.0358         &      0.0293         \\
            &    (0.0260)         &    (0.0245)         &    (0.0261)         &    (0.0245)         \\
Info $\times$ Shift Work&    -0.00533         &    -0.00394         &    -0.00109         &   -0.000533         \\
            &    (0.0244)         &    (0.0229)         &    (0.0246)         &    (0.0229)         \\
Info $\times$ Male&     -0.0146         &     -0.0186         &     -0.0144         &     -0.0179         \\
            &    (0.0239)         &    (0.0219)         &    (0.0245)         &    (0.0226)         \\
Info $\times$ Age&  -0.0000819         &    0.000668         &     0.00157         &     0.00204         \\
            &   (0.00478)         &   (0.00438)         &   (0.00483)         &   (0.00445)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&       19178         &       19178         &       19178         &       19178         \\
Individuals &         971         &         971         &         971         &         971         \\
Jobs        &        1124         &        1124         &        1124         &        1124         \\


==> raw_files/tab_belief_x_1_var.tex <==
\midrule
Current Wage&       0.751\sym{*}  &       0.750\sym{**} &       0.760\sym{*}  &       0.758\sym{*}  \\
            &     (0.123)         &     (0.107)         &     (0.123)         &     (0.121)         \\
Permanent   &       0.960         &       0.965         &       0.958         &       0.965         \\
            &    (0.0699)         &    (0.0736)         &    (0.0662)         &    (0.0688)         \\
Work From Home&       1.013         &       1.001         &       1.041         &       1.027         \\
            &     (0.115)         &     (0.116)         &     (0.123)         &     (0.121)         \\
Flexible Hours&       1.134         &       1.130         &       1.141         &       1.135         \\
            &    (0.0935)         &    (0.0930)         &    (0.0997)         &    (0.0900)         \\
Shift Work  &       1.030         &       1.022         &       1.074         &       1.057         \\
            &    (0.0841)         &    (0.0764)         &    (0.0915)         &    (0.0828)         \\
Male        &       1.029         &       1.033         &       1.091         &       1.100         \\
            &    (0.0849)         &    (0.0837)         &     (0.100)         &    (0.0895)         \\
Age         &       1.003         &       1.001         &       1.011         &       1.009         \\
            &    (0.0137)         &    (0.0131)         &    (0.0159)         &    (0.0151)         \\
Pay Information Effect&       1.992         &       1.368         &       1.881         &       1.263         \\
            &     (4.210)         &     (2.785)         &     (3.979)         &     (2.763)         \\
Info $\times$ Own Wage&       1.010         &       1.041         &       1.023         &       1.057         \\
            &     (0.213)         &     (0.206)         &     (0.218)         &     (0.225)         \\
Info $\times$ Permanent&       1.143         &       1.140         &       1.149         &       1.143         \\
            &     (0.116)         &     (0.118)         &     (0.127)         &     (0.113)         \\
Info $\times$ Work From Home&       1.156         &       1.146         &       1.148         &       1.138         \\
            &     (0.192)         &     (0.192)         &     (0.205)         &     (0.200)         \\
Info $\times$ Flexible Hours&       0.929         &       0.930         &       0.896         &       0.899         \\
            &     (0.115)         &     (0.105)         &     (0.109)         &     (0.110)         \\
Info $\times$ Shift Work&       0.933         &       0.944         &       0.867         &       0.882         \\
            &     (0.117)         &     (0.103)         &     (0.105)         &    (0.0973)         \\
Info $\times$ Male&       0.923         &       0.906         &       0.912         &       0.892         \\
            &     (0.105)         &    (0.0940)         &     (0.109)         &     (0.103)         \\
Info $\times$ Age&       0.959\sym{**} &       0.962\sym{**} &       0.958\sym{**} &       0.961\sym{**} \\
            &    (0.0191)         &    (0.0171)         &    (0.0177)         &    (0.0191)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&       19178         &       19178         &       19178         &       19178         \\
Individuals &         971         &         971         &         971         &         971         \\
Jobs        &        1124         &        1124         &        1124         &        1124         \\


==> raw_files/tab_belief_z_0.tex <==
\midrule
Permanent   &      0.0881\sym{***}&      0.0931\sym{***}&      0.0772\sym{***}&      0.0812\sym{***}\\
            &    (0.0212)         &    (0.0201)         &    (0.0160)         &    (0.0144)         \\
Work From Home&     0.00775         &      0.0198         &     0.00902         &      0.0211         \\
            &    (0.0336)         &    (0.0291)         &    (0.0277)         &    (0.0220)         \\
Shift Work  &      -0.126\sym{***}&      -0.125\sym{***}&      -0.117\sym{***}&      -0.113\sym{***}\\
            &    (0.0163)         &    (0.0150)         &    (0.0183)         &    (0.0163)         \\
Flexible Hours&      0.0649\sym{***}&      0.0605\sym{***}&      0.0465\sym{***}&      0.0434\sym{***}\\
            &    (0.0185)         &    (0.0178)         &    (0.0158)         &    (0.0141)         \\


==> raw_files/tab_belief_z_0_var.tex <==
\midrule
Permanent   &       0.813\sym{**} &       0.863         &       0.792\sym{**} &       0.844\sym{**} \\
            &    (0.0722)         &    (0.0778)         &    (0.0720)         &    (0.0715)         \\
Work From Home&       1.016         &       0.991         &       1.034         &       1.015         \\
            &     (0.133)         &     (0.124)         &     (0.125)         &     (0.120)         \\
Shift Work  &       1.094         &       1.110         &       1.090         &       1.112         \\
            &     (0.113)         &     (0.121)         &     (0.134)         &     (0.116)         \\
Flexible Hours&       0.910         &       0.901         &       0.896         &       0.881         \\
            &    (0.0873)         &    (0.0815)         &    (0.0877)         &    (0.0755)         \\


==> raw_files/tab_belief_z_0p.tex <==
\midrule
Amenity Value, Literature&       0.444\sym{***}&       0.449\sym{***}&       0.381\sym{***}&       0.387\sym{***}\\
            &    (0.0582)         &    (0.0546)         &    (0.0526)         &    (0.0449)         \\
Amenity Value, Subjective&       0.739\sym{***}&       0.748\sym{***}&       0.633\sym{***}&       0.640\sym{***}\\
            &    (0.0722)         &    (0.0665)         &    (0.0682)         &    (0.0588)         \\
Amenity Value, HCE&       0.672\sym{***}&       0.693\sym{***}&       0.576\sym{***}&       0.596\sym{***}\\
            &    (0.0897)         &    (0.0820)         &    (0.0782)         &    (0.0662)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        9466         &        9466         &        9466         &        9466         \\
Individuals &         480         &         480         &         480         &         480         \\
Jobs        &         994         &         994         &         994         &         994         \\


==> raw_files/tab_belief_z_0p_var.tex <==
\midrule
Amenity Value, Literature&       0.498\sym{**} &       0.524\sym{**} &       0.474\sym{**} &       0.492\sym{**} \\
            &     (0.151)         &     (0.140)         &     (0.158)         &     (0.147)         \\
Amenity Value, Subjective&       0.367\sym{**} &       0.393\sym{**} &       0.359\sym{**} &       0.376\sym{**} \\
            &     (0.155)         &     (0.163)         &     (0.159)         &     (0.147)         \\
Amenity Value, HCE&       0.327\sym{***}&       0.382\sym{**} &       0.307\sym{***}&       0.355\sym{**} \\
            &     (0.142)         &     (0.150)         &     (0.132)         &     (0.145)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        9466         &        9466         &        9466         &        9466         \\
Individuals &         480         &         480         &         480         &         480         \\
Jobs        &         994         &         994         &         994         &         994         \\


==> raw_files/tab_belief_z_1.tex <==
\midrule
Permanent   &      0.0881\sym{***}&      0.0931\sym{***}&           0         &           0         \\
            &    (0.0212)         &    (0.0201)         &         (.)         &         (.)         \\
Work From Home&     0.00775         &      0.0198         &           0         &           0         \\
            &    (0.0336)         &    (0.0291)         &         (.)         &         (.)         \\
Shift Work  &      -0.126\sym{***}&      -0.125\sym{***}&           0         &           0         \\
            &    (0.0163)         &    (0.0150)         &         (.)         &         (.)         \\
Flexible Hours&      0.0649\sym{***}&      0.0605\sym{***}&           0         &           0         \\
            &    (0.0185)         &    (0.0178)         &         (.)         &         (.)         \\
Pay Information Effect&      0.0235         &           0         &      0.0305\sym{**} &           0         \\
            &    (0.0165)         &         (.)         &    (0.0142)         &         (.)         \\
Info $\times$ Permanent&    -0.00507         &    -0.00808         &     -0.0111         &     -0.0157\sym{*}  \\
            &    (0.0134)         &    (0.0114)         &    (0.0111)         &   (0.00853)         \\
Info $\times$ PWork from Home&      0.0322\sym{*}  &      0.0306\sym{**} &      0.0291\sym{*}  &      0.0288\sym{**} \\
            &    (0.0180)         &    (0.0133)         &    (0.0170)         &    (0.0114)         \\
Info $\times$ Shift WorkPermanent&      0.0192         &     0.00738         &      0.0241         &     0.00987         \\
            &    (0.0157)         &    (0.0124)         &    (0.0151)         &    (0.0110)         \\
Info $\times$ Flexible Hours&    -0.00575         &    -0.00742         &     -0.0114         &     -0.0111         \\
            &   (0.00991)         &   (0.00792)         &   (0.00955)         &   (0.00742)         \\


==> raw_files/tab_belief_z_1_var.tex <==
\midrule
Permanent   &       0.813\sym{**} &       0.863         &                     &                     \\
            &    (0.0722)         &    (0.0778)         &                     &                     \\
Work From Home&       1.016         &       0.991         &                     &                     \\
            &     (0.133)         &     (0.124)         &                     &                     \\
Shift Work  &       1.094         &       1.110         &                     &                     \\
            &     (0.113)         &     (0.121)         &                     &                     \\
Flexible Hours&       0.910         &       0.901         &                     &                     \\
            &    (0.0873)         &    (0.0815)         &                     &                     \\
Pay Information Effect&       0.926         &                     &       0.960         &                     \\
            &     (0.109)         &                     &     (0.114)         &                     \\
Info $\times$ Permanent&       1.004         &       0.895         &       0.971         &       0.887         \\
            &     (0.117)         &     (0.107)         &     (0.113)         &     (0.100)         \\
Info $\times$ PWork from Home&       0.845         &       0.897         &       0.830         &       0.881         \\
            &     (0.137)         &     (0.148)         &     (0.138)         &     (0.128)         \\
Info $\times$ Shift WorkPermanent&       0.795         &       0.787\sym{*}  &       0.790         &       0.793\sym{*}  \\
            &     (0.116)         &     (0.109)         &     (0.117)         &     (0.108)         \\
Info $\times$ Flexible Hours&       0.912         &       0.959         &       0.912         &       0.976         \\
            &    (0.0833)         &    (0.0871)         &    (0.0929)         &    (0.0861)         \\


==> raw_files/tab_belief_z_1p.tex <==
\midrule
Amenity Value, HCE&       0.672\sym{***}&       0.693\sym{***}&           0         &           0         \\
            &    (0.0897)         &    (0.0820)         &         (.)         &         (.)         \\
Pay Information Effect&      0.0235         &           0         &      0.0317\sym{**} &           0         \\
            &    (0.0147)         &         (.)         &    (0.0131)         &         (.)         \\
Info $\times$ Amenity Value&     -0.0168         &     -0.0178         &     -0.0655         &     -0.0612         \\
            &    (0.0596)         &    (0.0482)         &    (0.0510)         &    (0.0379)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         \\
Job FE      &                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&       19178         &       19178         &       19178         &       19178         \\
Individuals &         971         &         971         &         971         &         971         \\
Jobs        &        1124         &        1124         &        1124         &        1124         \\


==> raw_files/tab_belief_z_1p_var.tex <==
\midrule
Amenity Value, HCE&       0.327\sym{***}&       0.382\sym{**} &                     &                     \\
            &     (0.142)         &     (0.150)         &                     &                     \\
Pay Information Effect&       0.896         &                     &       0.920         &                     \\
            &    (0.0884)         &                     &    (0.0964)         &                     \\
Info $\times$ Amenity Value&       0.949         &       0.737         &       0.831         &       0.716         \\
            &     (0.469)         &     (0.391)         &     (0.464)         &     (0.333)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         \\
Job FE      &                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&       19178         &       19178         &       19178         &       19178         \\
Individuals &         971         &         971         &         971         &         971         \\
Jobs        &        1124         &        1124         &        1124         &        1124         \\


==> raw_files/timeuse.tex <==
\hline
Pay Information Module&      -3.591\sym{***}&      -3.591\sym{***}&      -3.505\sym{***}\\
            &     (0.298)         &     (0.305)         &     (0.369)         \\
Second Module Taken&      -3.200\sym{***}&      -3.200\sym{***}&      -3.200\sym{***}\\
            &     (0.298)         &     (0.305)         &     (0.318)         \\
Treatment group&      -0.402         &      -0.375         &      -0.330         \\
            &     (0.771)         &     (0.849)         &     (0.805)         \\
\hline
Observations&        1410         &        1410         &        1410         \\
Individuals &         705         &         705         &         705         \\
Control Mean&       10.86         &       10.86         &       10.86         \\
Individual controls&                     &  \checkmark         &  \checkmark         \\
Job characteristics&                     &                     &  \checkmark         \\


==> raw_files/values1.tex <==
\hline
Value of Actual Effect&     -0.0012         &      0.0008         &     -0.0007         &     -0.0014\sym{*}  &     -0.0026         \\
                    &    (0.0015)         &    (0.0005)         &    (0.0006)         &    (0.0008)         &    (0.0020)         \\
Value of Expected Effect&      0.0006         &      0.0003         &      0.0007\sym{**} &      0.0004\sym{*}  &      0.0021\sym{**} \\
                    &    (0.0007)         &    (0.0003)         &    (0.0003)         &    (0.0002)         &    (0.0009)         \\
Value of Difference &     -0.0018         &      0.0004         &     -0.0014\sym{**} &     -0.0018\sym{**} &     -0.0046\sym{**} \\
                    &    (0.0016)         &    (0.0006)         &    (0.0007)         &    (0.0008)         &    (0.0022)         \\


==> raw_files/values2.tex <==
\hline
Value of Actual Effect&     -0.0009         &      0.0008         &     -0.0006         &     -0.0014\sym{*}  &     -0.0020         \\
                    &    (0.0011)         &    (0.0006)         &    (0.0005)         &    (0.0007)         &    (0.0017)         \\
Value of Expected Effect&      0.0005         &      0.0003         &      0.0006\sym{**} &      0.0004\sym{*}  &      0.0018\sym{**} \\
                    &    (0.0005)         &    (0.0003)         &    (0.0003)         &    (0.0002)         &    (0.0007)         \\
Value of Difference &     -0.0014         &      0.0005         &     -0.0011\sym{**} &     -0.0017\sym{**} &     -0.0038\sym{**} \\
                    &    (0.0012)         &    (0.0007)         &    (0.0005)         &    (0.0008)         &    (0.0018)         \\


==> raw_files/values3.tex <==
\hline
Value of Actual Effect&     -0.0006         &      0.0006         &     -0.0013         &     -0.0013\sym{*}  &     -0.0026         \\
                    &    (0.0008)         &    (0.0004)         &    (0.0012)         &    (0.0007)         &    (0.0018)         \\
Value of Expected Effect&      0.0003         &      0.0003         &      0.0014\sym{**} &      0.0003\sym{*}  &      0.0023\sym{***}\\
                    &    (0.0004)         &    (0.0002)         &    (0.0006)         &    (0.0002)         &    (0.0008)         \\
Value of Difference &     -0.0009         &      0.0003         &     -0.0027\sym{**} &     -0.0016\sym{**} &     -0.0049\sym{**} \\
                    &    (0.0008)         &    (0.0005)         &    (0.0013)         &    (0.0007)         &    (0.0020)         \\


==> raw_files/valuesA.tex <==
Value of Pay Information Effect&     -0.0001         &      0.0002         &     -0.0015         &     -0.0016\sym{*}  \\
                    &    (0.0024)         &    (0.0009)         &    (0.0010)         &    (0.0010)         \\
Value of Expected Effect&      0.0012         &      0.0006         &      0.0014\sym{**} &      0.0007\sym{*}  \\
                    &    (0.0013)         &    (0.0005)         &    (0.0006)         &    (0.0004)         \\
Value of Difference &     -0.0013         &     -0.0004         &     -0.0028\sym{**} &     -0.0024\sym{**} \\
                    &    (0.0027)         &    (0.0010)         &    (0.0011)         &    (0.0010)         \\


==> raw_files/valuesB.tex <==
Value of Pay Information Effect&     -0.0001         &      0.0002         &     -0.0028         &     -0.0015\sym{*}  \\
                    &    (0.0012)         &    (0.0007)         &    (0.0019)         &    (0.0009)         \\
Value of Expected Effect&      0.0006         &      0.0005         &      0.0026\sym{**} &      0.0006\sym{*}  \\
                    &    (0.0007)         &    (0.0004)         &    (0.0011)         &    (0.0003)         \\
Value of Difference &     -0.0007         &     -0.0003         &     -0.0054\sym{**} &     -0.0021\sym{**} \\
                    &    (0.0014)         &    (0.0008)         &    (0.0022)         &    (0.0009)         \\


==> raw_files/valuesC.tex <==
Value of Pay Information Effect&     -0.0001         &      0.0002         &     -0.0012         &     -0.0016\sym{*}  \\
                    &    (0.0018)         &    (0.0010)         &    (0.0008)         &    (0.0009)         \\
Value of Expected Effect&      0.0009         &      0.0007         &      0.0011\sym{**} &      0.0007\sym{*}  \\
                    &    (0.0010)         &    (0.0006)         &    (0.0005)         &    (0.0004)         \\
Value of Difference &     -0.0010         &     -0.0004         &     -0.0023\sym{**} &     -0.0023\sym{**} \\
                    &    (0.0020)         &    (0.0012)         &    (0.0009)         &    (0.0010)         \\
\hline
Individuals&         705         &         705         &         705         &         705         \\


==> raw_files/willingness_to_pay.tex <==
\midrule
Permanent           &       0.173\sym{***}&       0.164\sym{***}&       0.107\sym{***}\\
                    &    (0.0240)         &    (0.0105)         &   (0.00247)         \\
Work From Home      &       0.130\sym{***}&       0.105\sym{***}&      0.0728\sym{***}\\
                    &    (0.0120)         &   (0.00720)         &   (0.00220)         \\
Shift Work          &      -0.127\sym{***}&     -0.0761\sym{***}&      -0.188\sym{***}\\
                    &   (0.00700)         &    (0.0125)         &   (0.00474)         \\
Flexible Hours      &       0.184\sym{***}&      0.0606\sym{***}&      0.0634\sym{***}\\
                    &    (0.0140)         &   (0.00513)         &   (0.00185)         \\
Travel Time (30 mins)&      -0.150\sym{***}&      -0.167\sym{***}&      -0.128\sym{***}\\
                    &    (0.0190)         &   (0.00542)         &   (0.00293)         \\
\midrule
Individuals         &                     &         854         &         854         \\


==> raw_files/wtp_gender.tex <==
\hline
Permanent   &       0.107\sym{***}&       0.123\sym{***}&       0.109\sym{***}&       0.185\sym{***}\\
            &   (0.00473)         &    (0.0148)         &   (0.00339)         &    (0.0159)         \\
Work From Home&      0.0710\sym{***}&      0.0786\sym{***}&      0.0752\sym{***}&       0.121\sym{***}\\
            &   (0.00413)         &    (0.0107)         &   (0.00300)         &    (0.0106)         \\
Shift Work  &      -0.203\sym{***}&     -0.0779\sym{***}&      -0.193\sym{***}&     -0.0925\sym{***}\\
            &   (0.00908)         &    (0.0216)         &   (0.00689)         &    (0.0182)         \\
Flexible Hours&      0.0584\sym{***}&      0.0543\sym{***}&      0.0665\sym{***}&      0.0789\sym{***}\\
            &   (0.00364)         &   (0.00829)         &   (0.00249)         &   (0.00825)         \\
Travel Time (30 mins)&      -0.141\sym{***}&      -0.170\sym{***}&      -0.128\sym{***}&      -0.171\sym{***}\\
            &   (0.00542)         &   (0.00888)         &   (0.00433)         &   (0.00778)         \\
\hline
Observations&         226         &        9240         &         516         &       20800         \\


==> raw_new/tab_belief_x_0.tex <==
\midrule
Current Wage&       0.120\sym{***}&       0.118\sym{***}&       0.117\sym{***}&       0.115\sym{***}\\
            &    (0.0411)         &    (0.0385)         &    (0.0404)         &    (0.0379)         \\
Permanent   &     0.00758         &     0.00239         &     0.00730         &    0.000895         \\
            &    (0.0209)         &    (0.0193)         &    (0.0209)         &    (0.0193)         \\
Work From Home&     0.00653         &    -0.00806         &      0.0128         &    -0.00328         \\
            &    (0.0331)         &    (0.0305)         &    (0.0336)         &    (0.0307)         \\
Flexible Hours&     -0.0315         &     -0.0258         &     -0.0298         &     -0.0254         \\
            &    (0.0232)         &    (0.0212)         &    (0.0235)         &    (0.0214)         \\
Shift Work  &    -0.00736         &     -0.0116         &    -0.00748         &     -0.0114         \\
            &    (0.0216)         &    (0.0200)         &    (0.0215)         &    (0.0198)         \\
Male        &      0.0614\sym{***}&      0.0616\sym{***}&      0.0682\sym{***}&      0.0687\sym{***}\\
            &    (0.0219)         &    (0.0198)         &    (0.0235)         &    (0.0212)         \\
Age         &     0.00113         &    0.000199         &   -0.000907         &    -0.00195         \\
            &   (0.00422)         &   (0.00391)         &   (0.00464)         &   (0.00433)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        6879         &        6879         &        6879         &        6879         \\
Individuals &         353         &         353         &         353         &         353         \\
Jobs        &         898         &         898         &         898         &         898         \\


==> raw_new/tab_belief_x_0_var.tex <==
\midrule
Current Wage&       0.734         &       0.723         &       0.760         &       0.753         \\
            &     (0.160)         &     (0.143)         &     (0.161)         &     (0.153)         \\
Permanent   &       0.960         &       0.957         &       0.954         &       0.956         \\
            &    (0.0827)         &    (0.0827)         &    (0.0877)         &    (0.0812)         \\
Work From Home&       0.984         &       0.960         &       1.023         &       0.996         \\
            &     (0.143)         &     (0.130)         &     (0.136)         &     (0.133)         \\
Flexible Hours&       1.090         &       1.087         &       1.098         &       1.088         \\
            &     (0.106)         &     (0.110)         &     (0.112)         &     (0.108)         \\
Shift Work  &       1.046         &       1.040         &       1.082         &       1.064         \\
            &    (0.0951)         &    (0.0961)         &    (0.0959)         &     (0.101)         \\
Male        &       1.107         &       1.098         &       1.178         &       1.179         \\
            &     (0.104)         &     (0.111)         &     (0.119)         &     (0.127)         \\
Age         &       1.001         &       0.999         &       1.010         &       1.006         \\
            &    (0.0159)         &    (0.0140)         &    (0.0167)         &    (0.0154)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        6879         &        6879         &        6879         &        6879         \\
Individuals &         353         &         353         &         353         &         353         \\
Jobs        &         898         &         898         &         898         &         898         \\


==> raw_new/tab_belief_x_1.tex <==
\midrule
Current Wage&       0.120\sym{***}&       0.118\sym{***}&       0.117\sym{***}&       0.115\sym{***}\\
            &    (0.0411)         &    (0.0385)         &    (0.0404)         &    (0.0379)         \\
Permanent   &     0.00758         &     0.00239         &     0.00730         &    0.000895         \\
            &    (0.0209)         &    (0.0193)         &    (0.0209)         &    (0.0193)         \\
Work From Home&     0.00653         &    -0.00806         &      0.0128         &    -0.00328         \\
            &    (0.0331)         &    (0.0305)         &    (0.0336)         &    (0.0307)         \\
Flexible Hours&     -0.0315         &     -0.0258         &     -0.0298         &     -0.0254         \\
            &    (0.0232)         &    (0.0212)         &    (0.0235)         &    (0.0214)         \\
Shift Work  &    -0.00736         &     -0.0116         &    -0.00748         &     -0.0114         \\
            &    (0.0216)         &    (0.0200)         &    (0.0215)         &    (0.0198)         \\
Male        &      0.0614\sym{***}&      0.0616\sym{***}&      0.0682\sym{***}&      0.0687\sym{***}\\
            &    (0.0219)         &    (0.0198)         &    (0.0235)         &    (0.0212)         \\
Age         &     0.00113         &    0.000199         &   -0.000907         &    -0.00195         \\
            &   (0.00422)         &   (0.00391)         &   (0.00464)         &   (0.00433)         \\
Pay Information Effect&       0.716         &       0.716         &       0.650         &       0.667         \\
            &     (0.522)         &     (0.481)         &     (0.524)         &     (0.484)         \\
Info $\times$ Own Wage&     -0.0656         &     -0.0672         &     -0.0638         &     -0.0670         \\
            &    (0.0521)         &    (0.0481)         &    (0.0522)         &    (0.0482)         \\
Info $\times$ Permanent&     -0.0466\sym{*}  &     -0.0477\sym{*}  &     -0.0500\sym{*}  &     -0.0497\sym{**} \\
            &    (0.0265)         &    (0.0245)         &    (0.0268)         &    (0.0247)         \\
Info $\times$ Work From Home&     -0.0323         &     -0.0144         &     -0.0434         &     -0.0246         \\
            &    (0.0407)         &    (0.0372)         &    (0.0416)         &    (0.0377)         \\
Info $\times$ Flexible Hours&      0.0558\sym{*}  &      0.0459\sym{*}  &      0.0519\sym{*}  &      0.0435         \\
            &    (0.0295)         &    (0.0274)         &    (0.0297)         &    (0.0273)         \\
Info $\times$ Shift Work&      0.0104         &      0.0117         &      0.0105         &      0.0120         \\
            &    (0.0277)         &    (0.0257)         &    (0.0280)         &    (0.0258)         \\
Info $\times$ Male&     -0.0276         &     -0.0321         &     -0.0334         &     -0.0371         \\
            &    (0.0277)         &    (0.0252)         &    (0.0284)         &    (0.0256)         \\
Info $\times$ Age&     0.00104         &     0.00190         &     0.00342         &     0.00416         \\
            &   (0.00534)         &   (0.00478)         &   (0.00576)         &   (0.00519)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&       13723         &       13723         &       13723         &       13723         \\
Individuals &         705         &         705         &         705         &         705         \\
Jobs        &        1067         &        1067         &        1067         &        1067         \\


==> raw_new/tab_belief_x_1_var.tex <==
\midrule
Current Wage&       0.734         &       0.723         &       0.760         &       0.753         \\
            &     (0.160)         &     (0.143)         &     (0.161)         &     (0.153)         \\
Permanent   &       0.960         &       0.957         &       0.954         &       0.956         \\
            &    (0.0827)         &    (0.0827)         &    (0.0877)         &    (0.0812)         \\
Work From Home&       0.984         &       0.960         &       1.023         &       0.996         \\
            &     (0.143)         &     (0.130)         &     (0.136)         &     (0.133)         \\
Flexible Hours&       1.090         &       1.087         &       1.098         &       1.088         \\
            &     (0.106)         &     (0.110)         &     (0.112)         &     (0.108)         \\
Shift Work  &       1.046         &       1.040         &       1.082         &       1.064         \\
            &    (0.0951)         &    (0.0961)         &    (0.0959)         &     (0.101)         \\
Male        &       1.107         &       1.098         &       1.178         &       1.179         \\
            &     (0.104)         &     (0.111)         &     (0.119)         &     (0.127)         \\
Age         &       1.001         &       0.999         &       1.010         &       1.006         \\
            &    (0.0159)         &    (0.0140)         &    (0.0167)         &    (0.0154)         \\
Pay Information Effect&       1.342         &       1.011         &       1.227         &       0.953         \\
            &     (3.717)         &     (2.860)         &     (3.525)         &     (2.606)         \\
Info $\times$ Own Wage&       1.043         &       1.067         &       1.053         &       1.075         \\
            &     (0.286)         &     (0.285)         &     (0.292)         &     (0.287)         \\
Info $\times$ Permanent&       1.109         &       1.128         &       1.125         &       1.135         \\
            &     (0.146)         &     (0.141)         &     (0.141)         &     (0.139)         \\
Info $\times$ Work From Home&       1.305         &       1.331         &       1.317         &       1.335         \\
            &     (0.267)         &     (0.261)         &     (0.258)         &     (0.281)         \\
Info $\times$ Flexible Hours&       0.945         &       0.942         &       0.901         &       0.905         \\
            &     (0.125)         &     (0.136)         &     (0.127)         &     (0.128)         \\
Info $\times$ Shift Work&       0.951         &       0.951         &       0.893         &       0.901         \\
            &     (0.126)         &     (0.130)         &     (0.117)         &     (0.129)         \\
Info $\times$ Male&       0.848         &       0.849         &       0.856         &       0.852         \\
            &     (0.113)         &     (0.127)         &     (0.113)         &     (0.124)         \\
Info $\times$ Age&       0.959\sym{**} &       0.961\sym{*}  &       0.960\sym{*}  &       0.962\sym{*}  \\
            &    (0.0201)         &    (0.0211)         &    (0.0206)         &    (0.0199)         \\
1.infotreatment#c.nojob&       0.680         &       0.695         &       0.661         &       0.691         \\
            &     (0.225)         &     (0.236)         &     (0.244)         &     (0.251)         \\
\midrule
Job FE      &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&       13723         &       13723         &       13723         &       13723         \\
Individuals &         705         &         705         &         705         &         705         \\
Jobs        &        1067         &        1067         &        1067         &        1067         \\


==> raw_new/tab_belief_z_0.tex <==
\midrule
Permanent   &      0.0915\sym{***}&      0.0994\sym{***}&      0.0778\sym{***}&      0.0840\sym{***}\\
            &    (0.0229)         &    (0.0215)         &    (0.0177)         &    (0.0155)         \\
Work From Home&      0.0110         &      0.0265         &     0.00652         &      0.0232         \\
            &    (0.0366)         &    (0.0297)         &    (0.0308)         &    (0.0229)         \\
Shift Work  &      -0.118\sym{***}&      -0.121\sym{***}&      -0.112\sym{***}&      -0.113\sym{***}\\
            &    (0.0171)         &    (0.0155)         &    (0.0195)         &    (0.0169)         \\
Flexible Hours&      0.0627\sym{***}&      0.0623\sym{***}&      0.0444\sym{**} &      0.0433\sym{***}\\
            &    (0.0191)         &    (0.0180)         &    (0.0172)         &    (0.0146)         \\


==> raw_new/tab_belief_z_0_var.tex <==
\midrule
Permanent   &       0.849\sym{*}  &       0.918         &       0.818\sym{**} &       0.886         \\
            &    (0.0781)         &    (0.0969)         &    (0.0793)         &    (0.0864)         \\
Work From Home&       1.015         &       1.014         &       1.042         &       1.051         \\
            &     (0.155)         &     (0.135)         &     (0.155)         &     (0.151)         \\
Shift Work  &       1.115         &       1.149         &       1.122         &       1.160         \\
            &     (0.129)         &     (0.145)         &     (0.161)         &     (0.156)         \\
Flexible Hours&       0.922         &       0.910         &       0.897         &       0.878         \\
            &     (0.102)         &    (0.0986)         &     (0.106)         &    (0.0975)         \\


==> raw_new/tab_belief_z_0p.tex <==
\midrule
Amenity Value, Literature&       0.562\sym{***}&       0.603\sym{***}&       0.475\sym{***}&       0.513\sym{***}\\
            &    (0.0782)         &    (0.0711)         &    (0.0680)         &    (0.0571)         \\
Amenity Value, Subjective&       0.696\sym{***}&       0.736\sym{***}&       0.592\sym{***}&       0.627\sym{***}\\
            &    (0.0720)         &    (0.0648)         &    (0.0692)         &    (0.0582)         \\
Amenity Value, HCE&       0.683\sym{***}&       0.734\sym{***}&       0.575\sym{***}&       0.623\sym{***}\\
            &    (0.0945)         &    (0.0845)         &    (0.0853)         &    (0.0701)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        6879         &        6879         &        6879         &        6879         \\
Individuals &         353         &         353         &         353         &         353         \\
Jobs        &         898         &         898         &         898         &         898         \\


==> raw_new/tab_belief_z_0p_var.tex <==
\midrule
Amenity Value, Literature&       0.452\sym{**} &       0.543         &       0.402\sym{**} &       0.478\sym{*}  \\
            &     (0.173)         &     (0.205)         &     (0.164)         &     (0.188)         \\
Amenity Value, Subjective&       0.420\sym{*}  &       0.455\sym{*}  &       0.380\sym{*}  &       0.402\sym{**} \\
            &     (0.200)         &     (0.196)         &     (0.193)         &     (0.170)         \\
Amenity Value, HCE&       0.383\sym{*}  &       0.469\sym{*}  &       0.332\sym{**} &       0.401\sym{*}  \\
            &     (0.196)         &     (0.215)         &     (0.173)         &     (0.200)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         \\
Survey round FE&                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&        6879         &        6879         &        6879         &        6879         \\
Individuals &         353         &         353         &         353         &         353         \\
Jobs        &         898         &         898         &         898         &         898         \\


==> raw_new/tab_belief_z_1.tex <==
\midrule
Permanent   &      0.0915\sym{***}&      0.0994\sym{***}&           0         &           0         \\
            &    (0.0229)         &    (0.0215)         &         (.)         &         (.)         \\
Work From Home&      0.0110         &      0.0265         &           0         &           0         \\
            &    (0.0366)         &    (0.0297)         &         (.)         &         (.)         \\
Shift Work  &      -0.118\sym{***}&      -0.121\sym{***}&           0         &           0         \\
            &    (0.0171)         &    (0.0155)         &         (.)         &         (.)         \\
Flexible Hours&      0.0627\sym{***}&      0.0623\sym{***}&           0         &           0         \\
            &    (0.0191)         &    (0.0180)         &         (.)         &         (.)         \\
Pay Information Effect&      0.0565\sym{***}&           0         &      0.0563\sym{***}&           0         \\
            &    (0.0203)         &         (.)         &    (0.0173)         &         (.)         \\
Info $\times$ Permanent&     -0.0162         &     -0.0166         &     -0.0141         &     -0.0184\sym{*}  \\
            &    (0.0172)         &    (0.0143)         &    (0.0144)         &    (0.0108)         \\
Info $\times$ PWork from Home&      0.0232         &      0.0192         &      0.0192         &      0.0173         \\
            &    (0.0214)         &    (0.0147)         &    (0.0207)         &    (0.0113)         \\
Info $\times$ Shift WorkPermanent&      0.0187         &   -0.000896         &      0.0245         &     0.00537         \\
            &    (0.0163)         &    (0.0135)         &    (0.0164)         &    (0.0126)         \\
Info $\times$ Flexible Hours&    -0.00972         &     -0.0174\sym{*}  &     -0.0139         &     -0.0178\sym{**} \\
            &    (0.0117)         &   (0.00944)         &    (0.0109)         &   (0.00844)         \\


==> raw_new/tab_belief_z_1_var.tex <==
\midrule
Permanent   &       0.849\sym{*}  &       0.918         &                     &                     \\
            &    (0.0781)         &    (0.0969)         &                     &                     \\
Work From Home&       1.015         &       1.014         &                     &                     \\
            &     (0.155)         &     (0.135)         &                     &                     \\
Shift Work  &       1.115         &       1.149         &                     &                     \\
            &     (0.129)         &     (0.145)         &                     &                     \\
Flexible Hours&       0.922         &       0.910         &                     &                     \\
            &     (0.102)         &    (0.0986)         &                     &                     \\
Pay Information Effect&       0.805\sym{*}  &                     &       0.855         &                     \\
            &    (0.0942)         &                     &     (0.118)         &                     \\
Info $\times$ Permanent&       1.082         &       0.964         &       1.034         &       0.934         \\
            &     (0.134)         &     (0.134)         &     (0.127)         &     (0.121)         \\
Info $\times$ PWork from Home&       0.764         &       0.777         &       0.753         &       0.776         \\
            &     (0.147)         &     (0.141)         &     (0.142)         &     (0.144)         \\
Info $\times$ Shift WorkPermanent&       0.809         &       0.775\sym{*}  &       0.784         &       0.757\sym{**} \\
            &     (0.128)         &     (0.120)         &     (0.134)         &     (0.107)         \\
Info $\times$ Flexible Hours&       0.885         &       0.931         &       0.886         &       0.942         \\
            &     (0.103)         &     (0.110)         &     (0.102)         &    (0.0989)         \\


==> raw_new/tab_belief_z_1p.tex <==
\midrule
Amenity Value, HCE&       0.683\sym{***}&       0.734\sym{***}&           0         &           0         \\
            &    (0.0945)         &    (0.0845)         &         (.)         &         (.)         \\
Pay Information Effect&      0.0548\sym{***}&           0         &      0.0587\sym{***}&           0         \\
            &    (0.0169)         &         (.)         &    (0.0151)         &         (.)         \\
Info $\times$ Amenity Value&     -0.0809         &     -0.0798         &     -0.0987         &     -0.0987         \\
            &    (0.0710)         &    (0.0557)         &    (0.0638)         &         (.)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         \\
Job FE      &                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&       13723         &       13723         &       13723         &       13723         \\
Individuals &         705         &         705         &         705         &         705         \\
Jobs        &        1067         &        1067         &        1067         &        1067         \\


==> raw_new/tab_belief_z_1p_var.tex <==
\midrule
Amenity Value, HCE&       0.383\sym{*}  &       0.469\sym{*}  &                     &                     \\
            &     (0.196)         &     (0.215)         &                     &                     \\
Pay Information Effect&       0.814\sym{*}  &                     &       0.840         &                     \\
            &    (0.0920)         &                     &     (0.102)         &                     \\
Info $\times$ Amenity Value&       1.012         &       0.813         &       0.923         &       0.788         \\
            &     (0.610)         &     (0.453)         &     (0.543)         &     (0.390)         \\
\midrule
Person FE   &                     &$\checkmark$         &                     &$\checkmark$         \\
Job FE      &                     &                     &$\checkmark$         &$\checkmark$         \\
Observations&       13723         &       13723         &       13723         &       13723         \\
Individuals &         705         &         705         &         705         &         705         \\
Jobs        &        1067         &        1067         &        1067         &        1067         \\

